Approximation Schemes for Geometric Knapsack for Packing Spheres and Fat Objects

We study the geometric knapsack problem in which we are given a set of $d$-dimensional objects (each with associated profits) and the goal is to find the maximum profit subset that can be packed non-overlappingly into a given $d$-dimensional (unit hypercube) knapsack. Even if $d=2$ and all input objects are disks, this problem is known to be \textsf{NP}-hard [Demaine, Fekete, Lang, 2010]. In this paper, we give polynomial time $(1+\varepsilon)$-approximation algorithms for the following types of input objects in any constant dimension $d$: - disks and hyperspheres, - a class of fat convex polygons that generalizes regular $k$-gons for $k\ge 5$ (formally, polygons with a constant number of edges, whose lengths are in a bounded range, and in which each angle is strictly larger than $\pi/2$), - arbitrary fat convex objects that are sufficiently small compared to the knapsack. We remark that in our \textsf{PTAS} for disks and hyperspheres, we output the computed set of objects, but for a $O_\varepsilon(1)$ of them, we determine their coordinates only up to an exponentially small error. However, it is unclear whether there always exists a $(1+\varepsilon)$-approximate solution that uses only rational coordinates for the disks' centers. We leave this as an open problem that is related to well-studied geometric questions in the realm of circle packing.

==> 4spheres-rational.tex <==

\section{Spheres with only rational coordinates}
\label{sec:rational}

\begin{figure}
	\begin{center}
		\includegraphics[width=10cm]{Figures/3-bin-generation.pdf}
		\caption{Dividing augmented packing $P$ into three unit bin packings $B_1,B_2,B_3$}
		\label{fig:partition-img-3bins}
	\end{center}
	
\end{figure}


As discussed earlier, for the geometric knapsack
problem with circles or $d$-dimensional hyperspheres, it is not clear
that there always exists an optimal or $(1+\eps)$-approximate solution
that uses only rational coordinates.

We show that for arbitrary dimension, there is a polynomial time $3$-approximation
algorithm  that outputs a solution with rational coordinates only (with
a polynomial number of bits). In particular, this implies that there \emph{exists}
always a solutions with
rational coordinates that is by at most a factor $3$ worse than
the optimal solution with arbitrary coordinates.


\begin{theorem}[$\star$]
	Let $d\in\mathbb{N}$ be a constant. For the geometric knapsack problem
	with $d$-dimensional hyperspheres, there is a polynomial time $3$-approximation
	algorithm.
\end{theorem}


\noindent \emph{Proof sketch.} We first begin with a packing $P$ in the augmented hypercube of dimensions $(1+\eps)\times 1 ...\times 1$ such that the total packed profit is at least $w(\OPT)$, by using \Cref{extended-wowa}. Any hypersphere in the hypercube with diameter \(\geqslant 1-\eps\), we call as huge hypersphere and further prove that there can be atmost one huge hypersphere in any feasible packing. This property essentially helps us to partition the hyperspheres in the bin into three types of hypersphers depending upon their relative position with respect to $\eps$-augmenting planes $\ell$ and $\ell'$ which are perpendicular to the augmented side of the hypercube of length $1+\eps$ and are at a distance of $\eps$ from the left face and right face, respectively (see \Cref{fig:partition-img-3bins}). We pack these three types of hyperspheres in three separate unit hypercube and return the one of maximum weight with weight at least \(\frac{w(\OPT)}{3}\). Details of this result can be found in \Cref{sec:appendix-3-apx}.


\begin{figure}
	\begin{center}
		\includegraphics[width=10cm]{Figures/hypersphere_bin_generation.pdf}
		\caption{Dividing augmented packing $P$ into two unit bin packings $B_1$ and $B_2$ with the help of $\eps$-slab $D$}
		\label{fig:partition-img-2bins}
	\end{center}
	
\end{figure}


We improve upon it for any dimension
$d\leqslant8$, to give a $2+\eps$-approximation
algorithm (again, using only rational coordinates with a polynomially bounded number of bits).
\begin{restatable}[\emph{$\star$}]{theorem}{geometricknapsacktheoremapx}
	\label{geometric-knapsack-theorem}
	Let $d\leqslant8$ be a constant. For the geometric knapsack problem with $d$-dimensional hyperspheres, there is a polynomial time $(2+\eps)$-approximation algorithm.
\end{restatable}

\noindent \emph{Proof sketch.} For dimension \(d \leqslant 8\), we show that we do not need to pack huge hypersphere in a separate bin. In case there is no huge hypersphere in our packing, we can partition the set of hyperspheres in two separate bins. In the case there is a huge hypersphere, we prove the existence of a empty \(\eps\)-strip in the middle of the bin which restricts the dimension to \(d \leqslant 8\). This
empty \(\eps\)-strip we can merge the hypersphers in bin $B_1$ and $B_3$ (see \Cref{fig:partition-img-3bins}) in a bin $B_1$  (see \Cref{fig:partition-img-2bins}) and all the packed hyperspheres can be packed in two unit hypercubes. We return the best of the two packings which ensure a profit of \(\frac{(1-\eps)}{2}w(\OPT)\).
Details of this result can be found in \Cref{sec:appendix-2-apx}.


==> 4weighted.tex <==
\section{Spheres with only rational coordinates}
\label{sec:weighted}

In the problem $\mathsf{d-CSK}$, we are given a set $\mathcal{C}$ of weighted $d$-dimensional hyperspheres and we wish to pack maximum profit into a unit bin.
For a constant $\eps>0$, we first get a packing $P$ into the augmented bin of size \((1+\eps) \times ... \times 1\).
We propose a $3$-approximation algorithm that works for all dimensions and improve upon it to give a $(2+\eps)$-approximation algorithm that works only for dimensions $d\leqslant 8$.

\subsection{Augmented Optimal Packing}

Let $\OPT$ be an optimal solution, $\C_{\OPT}$ be the spheres in $\OPT$, and $w(\OPT)$ be the optimal weight.

\begin{comment}
\begin{restatable}{lem}{mylemmaone}
	\label{mylemma}
	I claim that $1+1=2$.
\end{restatable}
\end{comment}

\begin{restatable}{theorem}{extendedwoawabs}
	\label{extended-wowa}
	Let $\mathcal{C}$ be an instance of the $\mathsf{d-CSK}$ problem and \(\eps \geqslant 0\) be a small enough constant. There is a polynomial time algorithm that finds a packing $P$ of a subset \(\mathcal{C}^'\subseteq \mathcal{C}\) in an augmented knapsack of size \((1+\eps) \times \cdots \times 1\) such that \(p(\mathcal{C}^')\geqslant w(\OPT) \), where $\OPT$ is the optimal solution.
\end{restatable}
\begin{proof}
	
	We use the shifting strategy mentioned in section \Cref{lem:shifting} with $\rho_{k,1}= \eps^k$ to get set of hyperspheres $\mathcal{C}_M$ with a total weight less than $\eps \cdot w(\OPT)$ and radius between $\eps^{\tau_1-1}$ and $\eps^{\tau_1}$ for some $\tau_1<1/\eps$. Now we use the shifting strategy again on the set $\mathcal{C}_M$ but for volume instead of weight. With $\rho_{k,2} =\eps^{\frac{k\tau_1 - 1}{k}}$, there is a $\tau_2 \leqslant 1/\eps$ as the total volume of $\mathcal{C}_M$ is at most 1, such that we can get a set of hyperspheres $\mathcal{C}_{removed}$ such that it has a total profit less than $\eps \cdot w(\OPT)$, total volume less than $\eps$, and all radii between $\rho_{\tau_2-1, 2}$ and $\rho_{\tau_2, 2}$. 
	
	Using the algorithm provided in \cite{MiyazawaWAOA} for a suitable constant $\eps'$ such that the set of medium hyperspheres described in \Cref{lem:shifting} removed is that same as the $\mathcal{C}_{removed}$ above, we get a packing of $w(\OPT) - w(\mathcal{C}_{removed})$ total weight in a bin of size \((1+\eps') \times \cdots \times 1\). Now, notice that $\mathcal{C}_{removed}$ can be packed into a unit slab of width $O(\eps)$ using the $\mathtt{NFDH}$ algorithm explained in \cite{NFDH}. Join this slab to our already augmented bin to get a further segmentation but a packing of $w(\OPT)$. Choose an $\eps''= \eps+\eps'$ to get our result.
\end{proof}
\subsection{$3$-approximation algorithm for all dimensions $d$}

 Using theorem \ref{extended-wowa}, we get a packing $P$ in the augmented hypercube of dimensions $(1+\eps)\times 1 ...\times 1$ such that the total packed profit is at least $w(\OPT)$.



\begin{figure}[ht]
	\begin{center}
		\includegraphics[width=10cm]{Figures/3-bin-generation.pdf}
		\caption{Dividing augmented packing $P$ into three unit bin packings $B_1,B_2,B_3$}
		\label{fig:partition-img}
	\end{center}
	
\end{figure}

Call two $\eps$-augmenting planes $\ell$ and $\ell'$ which are perpendicular to the augmented side of the hypercube of length $1+\eps$ and are at a distance of $\eps$ from the left face and right face respectively. Let us define three types of hyperspheres in the packing $P$ obtained above in the augmented hypercube as shown in Figure \ref{fig:partition-img}. Define \textit{type 1 hyperspheres} to be the hyperspheres in $P$ which are completely inside the $(1-\eps)\times 1 \times ... \times 1$ $d$-dimensional slab to the left of $\ell$ and to the right of $\ell'$, \textit{type 2 hyperspheres} to be the hyperspheres in $P$ which intersect $\ell$, \textit{type 2' hyperspheres} to be the hyperspheres in $P$ which intersect $\ell'$, and finally \textit{type 3 and 3' hyperspheres} to be the hyperspheres in $P$ which are completely contained inside the '$\eps$-slab' of dimensions $\eps\times 1 \times ... \times 1$ to the right of $\ell$ and left of $\ell'$ respectively. We now prove that for small values of $\eps$, there can be at most one \textit{huge} hypersphere that intersects both $\ell$ and $\ell'$. Since the distance between the planes $\ell$ and $\ell'$ is $1-\eps$, a \textit{huge} hypersphere must have a diameter of at least $1-\eps$ to intersect both $\ell,\ell'$.

\begin{restatable}{lemma}{nextradabs}
	\label{nextrad}
	If a huge hypersphere i.e., a hypersphere with a diameter greater than or equal to $1-\eps$ is packed in the augmented bin of dimensions $(1+\eps)\times 1 \times \ldots \times 1$, then the radius of the second biggest hypersphere is at most $\frac{1}{2}+\frac{1}{d-1}+\eps\left(\frac{1}{2} + \frac{2}{d-1}\right) -\sqrt{\frac{(1+\eps)^2}{(d-1)^2}+\frac{1-\eps^2}{d-1}}$.
\end{restatable}
\begin{proof}
	The radius of the next hypersphere will be the biggest when the the diameter of the \textit{huge} sphere is exactly $1-\eps$ and is pushed to a corner and the next hypersphere of radius $r$ is pushed to the diagonally opposite corner in the augmented bin. We claim that $r$ satisfies the form given above exactly. We use the pythagorean theorem in $d$-dimensions repeatedly. The situation is described clearly in two dimensions in Figure \ref{hypersphere}.
	%\newpage
	\begin{figure}[ht]
		\centering
		\begin{tikzpicture}[scale=0.5]
		\coordinate (a) at (0,0);
		\coordinate (b) at (12,0);
		\coordinate (c) at (0,9);
		\coordinate (d) at (12,9);
		\coordinate (e) at (2,0);
		\coordinate (f) at (12-4.29,0);
		\draw (0,0) rectangle (12,9);
		\draw (2,2) circle (2cm);
		x=4;
		\draw (12-4.29,9-4.29) circle (4.29 cm);
		\draw[dashed] (2,2) -- (12,2);
		\draw [dashed] (12-4.29,0) -- (12-4.29,9);
		\draw [dashed] (2,2) -- (12-4.29,9-4.29);
		\draw [dashed] (2,0) -- (2,2);
		\draw [dashed] (0,2) -- (2,2);
		\draw (2,2) circle (2cm);
		\node[above left] at (2,2) {$O_2$};
		\node[above left] at (12-4.29,9-4.29) {$O_1$};
		\node[above left] at (12-4.29,2) {$P$};
		\draw[<->] ([yshift=-0.3cm]f) -- ([yshift=-0.3cm]b) node[midway, below]{$(1-\eps)/2$};
		\draw[<->] ([yshift=-0.3cm]a) -- ([yshift=-0.3cm]e) node[midway, below]{$r$};
		\label{Figure 4}
		\end{tikzpicture}
		\caption{Worst case scenario for second biggest sphere in two dimensions.}
		\label{hypersphere}
	\end{figure}
	%\newpage
	% \\\includegraphics[width=10cm]{Images/hypersphere.jpeg}
	
	Let a huge circle of the minimum diameter $1-\eps$ be pushed to the rightmost corner of the augmented box centered at $O_1$. We try and fit a circle of radius $r$ in the bottom-left corner of the box centered at $O_2$. We notice that in 2 dimensions, $O_1 O_2 P$ forms a right triangle. $O_2 P= 1+\eps - r - (1-\eps)/2$, $O_1 P = 1 - r - (1-\eps)/2$, and $O_1 O_2 = r + (1-\eps)/2$. Applying Pythagorean theorem in two dimensions, we get $r=\frac{3}{2} (1+\eps) - \sqrt(2+3\eps)$. In d-dimensions, this generalises to $r= \frac{1}{2}+\frac{1}{d-1}+\eps( \frac{1}{2} + \frac{2}{d-1}) -\sqrt{\frac{(1+\eps)^2}{(d-1)^2}+\frac{1-\eps^2}{d-1}}$ and we are done.
\end{proof}

\begin{restatable}{lemma}{uniqhugeaabs}
	\label{uniqhuge}
	For any $0 < \eps \leqslant 1/2d^2$ for all $d \geqslant 2$, there can be at most one hypersphere in $P$ with a diameter larger than $1-\eps$.
\end{restatable}
\begin{proof}
	We always get at most one \textit{huge} hypersphere if the radius calculated in the lemma \ref{nextrad} is always less than $(1-\eps)/2$. We show that such an $\eps>0$ can always exist regardless of $d$.
	\[\frac{1}{2}+\frac{1}{d-1}+\eps( \frac{1}{2} + \frac{2}{d-1}) -\sqrt{\frac{(1+\eps)^2}{(d-1)^2}+\frac{1-\eps^2}{d-1}} \leqslant (1-\eps)/2 \]
	Analytically solving the quadratic equation, it always holds for \[\eps \leqslant \frac{\sqrt{d^3+3d^2-4d+1}-d}{d^2+3d-1} \leqslant \frac{1}{2d^2}\] where the bound is always positive for all $d \geqslant 2$.
\end{proof}

\begin{restatable}{theorem}{apxtheoremabs}
	\label{3apx}
	There is a polynomial time $3$-approximation algorithm for the $\mathsf{d-CSK}$ problem.
\end{restatable}
\begin{proof}
	We show that for values of $\eps<1/2d^2$ as given in lemma \ref{uniqhuge} we can always partition the augmented bin packing $P$ into three separate packings into unit hypercube bins $B_1, B_2,$ and $B_3$. Let the unique huge hypersphere that intersects both $\ell$ and $\ell'$ be called $C_{huge}$ and remove $C_{huge}$ from all other types of hyperspheres in $P$ as defined earlier. If there is no \textit{huge} hypersphere, then ignore this step. Now note that the set of type 1, type 2, type 3, type 2', type 3', and $C_{huge}$ form a partition of the hyperspheres in $P$.  
	\\We first pack $B_1$ using the same structure as in $P$ with hyperspheres of type 3' and type 2'. This is possible as no hypersphere of type 2' can intersect $\ell$ and we can simply remove the $\eps$-slab to the right of $\ell'$ and we get our bin packing $B_1$. We then pack $B_3$ with hyperspheres of type 2, type 3, and type 1. We then pack the unique hypersphere $C_{huge}$ which has a diameter of at most 1 in a unit bin $B_2$. Note here that we needed to have at most one $C_{huge}$ as the bin width could have been more than 1 even though the huge hyperspheres themselves had a diameter less than 1. We then return the bin out of $B_1, B_2, B_3$ with the most profit.
	\\The running time of this algorithm is clearly polynomial as the we get the augmented packing from lemma \ref{extended-wowa} in polynomial time and the partitioning takes linear time. 
	 Since we return the bin with the maximum weight, we return a instance of $\mathsf{d-CSK}$ with a profit of at least $\frac{1}{3} w(\OPT)$. 
\end{proof}

\subsection{$(2+\eps)$-approximation algorithm for \(d\leq 8\)}
The main goal of this section is to show that the packings we return for bins $B_1$ and $B_3$ in the $3$-approximation algorithms can in fact be packed into a single bin for $d\leqslant 8$. When there are no \textit{huge} hyperspheres with a diameter greater than $(1-\eps)$, a simple argument for packing in two bins can be made. Also, from lemma \ref{uniqhuge} we know that for small enough values of $\eps$, there can be at most one \textit{huge} hypersphere.

\begin{restatable}{lemma}{nohugelemmaapx}
	\label{nohuge}
	If there are no \textit{huge} hyperspheres with a diameter bigger than $1-\eps$, then the augmented bin packing $P$ can be partitioned into two unit bin packings $B_1$ and $B_2$.
\end{restatable}
\begin{proof}
	We partition using the same algorithm as in theorem \ref{3apx} into three unit bins. However the bin that contained the \textit{huge} hypersphere before is now completely empty, so we simply return the other two bins.
\end{proof}

If we have a unique \textit{huge} hypersphere $C_{huge}$, we again show that we can pack $P$ into two different unit bin packings $B_1$ and $B_2$. Let us define another $\eps$-slab $D$ which is parallel to $\ell$ and $\ell'$ and is situated exactly halfway between the two and has $\eps$-width. To use our strategy we need an "empty" $\eps$-slab $S$ in the middle of the augmented bin, which restricts the dimension to $d\leqslant 8$.

\begin{figure}[ht]
	\begin{center}
		\includegraphics[width=10cm]{Figures/hypersphere_bin_generation.pdf}
		\caption{Dividing augmented packing $P$ into two unit bin packings $B_1$ and $B_2$ with the help of $\eps$-slab $D$}
		\label{fig:partition-img-2}
	\end{center}
	
\end{figure}

\begin{restatable}{lemma}{mindistlemma}
	\label{mindist}
	For $\eps < 1/d^2.2^d$ and $d \leqslant 8$, the distance between any arbitrary type 2 hypersphere and any arbitrary hypersphere of type 2' is at least $\eps$.
\end{restatable}
\begin{proof}
	If the diameter of the hypersphere calculated in lemma \ref{nextrad} is smaller than $1/2 - \eps$, this is true as the distance between $\ell$ and $D$, $\ell'$ and $D$ is $1/2 - \eps$.   
	\[\frac{1}{2}+\frac{1}{d-1}+\eps( \frac{1}{2} + \frac{2}{d-1}) -\sqrt{\frac{(1+\eps)^2}{(d-1)^2}+\frac{1-\eps^2}{d-1}} \leq 1/4 - \frac{\eps}{2}\]
	This inequality holds true for some positive value of $\eps$ only for $d\leq 8$.  
\end{proof}

\begin{restatable}{theorem}{approxtheorem}
	There is a polynomial time $(2+\eps)$-approximation algorithm for $\mathsf{d-CSK}$ for dimension $d<8$ and $0<\eps<1/4d^2.5^{2d+3}$.
\end{restatable}
\begin{proof}
	We choose $\eps$ small enough from lemma \ref{uniqhuge} such that there can be at most one \textit{huge} hypersphere of diameter bigger than $1-\eps$. Now, if there are no hyperspheres in the augmented packing $P$ obtained from lemma \ref{extended-wowa} with a diameter bigger than $1-\eps$, we proceed to partition and pack $P$ into two augmented unit bins $B_1$ and $B_2$ using lemma \ref{nohuge}. 
	\\In the case where there is a unique \textit{huge} hypersphere, we choose $\eps$ small enough from lemma \ref{uniqhuge} such that type 2 and type 2' hyperspheres in $P$ leave an empty $\eps$-strip $D$ between them in the middle of the augmented bin. Now we pack the only huge hypersphere $C_{huge}$ and type 1 hyperspheres into $B_2$. We now can simply remove the strip $D$ and join the segments to get a unit bin packing $B_1$ of hyperspheres of types 2,3,2',3'.
	\\At the end we return packing out of $B_1,B_2$ with maximum weight. This algorithm is clearly polynomial as we get the augmented packing from lemma \ref{extended-wowa} in polynomial time and the partitioning takes linear time. The algorithm returns an instance of $\mathsf{d-CSK}$ of total weight at least of $\frac{(1-\eps)}{2}w(\OPT)$.
\end{proof}

==> 5conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}


==> 5unweighted.tex <==
\section{Unweighted Setting}
\label{sec:unweighted}

In this scenario, we study the problem of packing a subset with a maximum number of hyperspheres from a collection $\mathcal{C}$ of unit weight $d$-dimensional hyperspheres in a unit bin. We call this problem unweighted $\mathsf{d-CPK}$ and its two-dimensional version unweighted $\mathsf{CPK}$. We propose a $5/2$-approximation algorithm for unweighted $\mathsf{d-CPK}$ that works for all dimensions $d$ based on ideas from the last section. Next, we introduce a new  $5/3$-approximation algorithm specifically for the two-dimensional case i.e. unweighted $\mathsf{CPK}$.

\subsection{$5/2$-approximation algorithm in all fixed dimensions $d$}
We now solve the $d$-dimensional hypersphere packing problem when each hypersphere has unit weight. To do this, we show that given a set of at most three hyperspheres that can be packed in a unit hypercube, we can always return the packing with a simple heuristic. %The proof of this is added to the appendix.z%
\begin{lemma}
	\label{twopack}
	Given a set $Q$ of at most two $d$-dimensional hyperspheres, there is a constant time algorithm to determine whether all hyperspheres of $Q$ can be packed inside a unit $d$-dimensional hypercube, and to return a packing if it exists. 
\end{lemma}
\begin{proof}
	Given an optimal packing of at most two hyperspheres, we can always push them to diagonally opposite corners of the unit hypercube.
	
	Our algorithm to find a packing of $Q$ is to simply to pack one hypersphere in a corner so that it touches all sides incident on that corner and then, if possible, pack the other hypersphere on the diagonally opposite corner so that it touches all sides incident on that corner. Return this packing if it was possible to pack $Q$ in this way, otherwise return that $Q$ cannot be packed inside a unit hypercube.
\end{proof}

\begin{theorem}
	There is polynomial time $5/2$-approximation algorithm for unweighted d-CSK in all dimensions $d$.
\end{theorem}
\begin{proof}
	We again get a packing in an augmented bin of profit of at least $w(\OPT)$ using the algorithm from lemma \ref{extended-wowa} for $\eps< 1/5^{2d+3}$. We then distinguish our algorithm between three parts depending on the value of $w(\OPT)$.
	
	Firstly, we can pack one hypersphere trivially and we can pack two hyperspheres using lemma \ref{twopack} for $2\leq w(\OPT)\leq 5$. 
	
	Next, when $6 \leq w(\OPT)$, we restrict $\eps<1/2d^2$ according to the bound in lemma \ref{uniqhuge} which guarantees us that for all $d$, there is only at most one hypersphere with a diameter greater than $1-\eps$. We then kill off this unique \textit{huge} hypersphere if it exists. We then apply the algorithm from lemma \ref{nohuge} as there is no \textit{huge} hypersphere and split our augmented packing into two packings into unit bins. We then return the bin with the larger weight. Note that we return at packing of at least $\lceil \frac{w(\OPT)-1}{2} \rceil$ hyperspheres. This always returns an output better than $2/5 \cdot w(\OPT)$ for $w(\OPT)\geq 6$. Combining the two cases, we get our result.
	
\end{proof}
\begin{comment}
	content...

\subsection{5/3-approximation algorithm for two dimensions}

In this section we attempt to get a 5/3-approximation algorithm for the unweighted $\mathsf{CSK}$ problem, i.e. the unweighted two-dimensional case of circle knapsack packing into a square. We begin by proving structural lemmas and then finally arrive at our algorithm.

\begin{lemma}
	\label{threepack}
	Given a set $Q$ of at most three $2$-dimensional circles, there is a constant time algorithm to determine whether all circles of $Q$ can be packed inside a unit square, and to return a packing if it exists. 
\end{lemma}
\begin{proof}
	%The idea is to first show that in any such packing, one circle can always be pushed to a corner. We can prove this combinatorially. Then the other two circles can be packed easily.%
	If the set \(Q\) contains only 1 circle, then if the radius of the circle is \(\leq \frac{1}{2}\), then we can always pack it with it's center overlapping with the center of the unit bin.
	
	If the set \(Q\) contains 2 circles, then we can pack the one circle at a corner touching two of the adjacent bin sides. Then we can pack the other circle at a diagonally opposite corner similarly touching two of the adjacent sides. If this strategy fails to produce a valid packing, then no such packing exists
	
	For the case, when the set \(Q\) contains 3 circles, then we show that all the possible valid packing can be modified to have a particular regular structure and we exhaust all of these possibilities to find out a feasible packing or conclude that no such packing exists.
	
	Suppose, the circles be \(Q=\{C_1,C_2,C_3\}\) and there is a valid packing named \(P\) of \(Q\) in a unit bin . We first consider a rectangular bin \(B\) whose each of the four sides touch at least one of the three circle. These is essentially the rectangle with the smallest side lengths which inscribe all the 3 circles. Firstly we note that there are only 3 circles and 4 sides of the rectangle which implies that at least one circle must touch two adjacent sides of \(B\). Without loss of generality we can assume that \(C_1\) is a circle which touch two adjacent sides of the bin \(B\). If there are more than 1 circle which touch two adjacent sides, then we consider the one with the smallest radius. Now, we consider the corner which has two of it's adjacent sides touched by \(C_1\) and name this corner point \(A^'\). We translate the bin \(B\) along with the circles in \(Q\) with their relative positions maintained inside the bin so that \(A^'\) overlaps with the it's nearest corner point \(A\) in the unit bin. After this step, we have \(C_1\) touching two of the adjacent sides of the unit bin. Depending on the relative ratio of the radius of \(C_2\) and \(C_3\) with \(C_1\), we can either translate each of \(C_2\) and \(C_3\) such that they either touch (i) two of the sides of the unit bin or (ii) one side of the unit bin and the circle \(C_1\). In both of the cases we have the position of the center of \(C_2\) and \(C_3\) deterministic depending upon which sides of the bin they touch. Now that we have shown this structural property for the feasible packing of set \(Q\), in order to decide if all the circles in \(Q\) can be packed in the unit bin we proceed as follows. For each \(i=1,2,3\) we pack the circle \(C_i\) in a corner \(A\) of the bin. For the other two circles, we try to pack them exhausting both of the cases described above for each of the circle. If any of the cases returns us a feasible packing we have found one feasible packing for \(Q\). Otherwise, we note that no feasible packing exist.
\end{proof}

%\label{greedyNFDR_section}

In the paper \cite{NFDH}, the authors consider the two-dimensional packing problem for packing squares into rectangles and propose a next fit decreasing height algorithm. We trivially extend their work for packing two dimensional circles with a bounded radius and unit weight into a unit square as \(\mathtt{NFDR}\) (Next fit decreasing radius algorithm), more formally stated as the lemma below.

\begin{lemma}
	\label{NFDR}
	Given a set of two-dimensional circles $Q$ such that each circle in $Q$ has a radius smaller than $\mu$, the
	\(\mathtt{NFDR}\) strategy packs an area of at least $\frac{\pi}{4}(1-4\mu)$ in a unit square.
\end{lemma}
\begin{proof}
	Draw a axis parallel bounding box over each of the circles we need to pack and pack this effective set of squares using the NFDH algorithm. In the paper \cite{NFDH} the NFDH algorithm produces the following guarantee, ``a set of squares $S$ with sidelengths $\leqslant \delta.$ If NFDH cannot place any square in a rectangle $R := r_1 \times r_2$, where $r_1, r_2 \geqslant\delta$, then total wasted space is less than or equal to $ \delta(r_1 + r_2)$.'' In our case, \(r_1=1,\) and  \(r_2= 1\) and \(\delta=2\mu.\) So, we get that total wasted space is less than or equal to \(4\mu\). Hence, we pack an area of \(1-4\mu\) at least. But, since we enclosed each circle with a square, we end up losing a fraction \(\frac{\pi}{4}\) of the area. Hence, finally we pack at least an area of \(\frac{\pi}{4}(1-4\mu).\)
\end{proof}

However, we generalise this for set of circles with unit weights with bounded radius $\leq \mu$. The appropriate modification to the problem is for us to have to pack a subset of circles $S'$ from a given set of circles $S$ with radii less than or equal to $\mu$ such that the number of circles that is packed is maximum. Let us call the following strategy $\mathtt{greedyNFDR}$:

We first sort all the circles in increasing order of their radius and declare a empty set $T$. We keep choosing the circles starting from the first circle and it to $T$ until we run out of circles or on adding a new circle to $T$, the sum of area of all the circles in $T$ exceeds $\frac{\pi}{4}(1-4\mu)$. Unless we run out of circles in constructing $T$, we can always construct $T$ with sum of area of circles in $T$ at least $\frac{\pi}{4}(1-4\mu)-\pi\mu^2$ since all the circles in $S$ have radius $\leq \mu$.

\begin{lemma}[{\(\mathtt{greedyNFDR}\)}]
	\label{greedyNFDR_lemma}
	The $\mathtt{greedyNFDR}$ strategy for circles with radii $\leq \mu$ and unit profit packs at least $\frac{\pi}{4}(1-4\mu)-\pi\mu^2$ fraction of circles that can be packed in the optimal packing of the square knapsack. 
\end{lemma}

\begin{proof}
	Let us order the circles in $S$ in increasing order of radius as \(S=\{c_1,c_2,c_3,...,c_n\}\). Suppose that the circle is able to pack a subset \(S_{\text{packed}}=\{c_1,c_2,...,c_s\}\) of size s where each circle has radius \(\leq r_{s}\) and is unable to pack the circles \(S_{\text{unpacked}}=\{c_{s+1},c_{s+2},...,c_n\}\) where each circles has radius \(\geq r_{s+1}\ \geq r_{s}\).  Note that if the total area of circles in $S$ is less than \(\frac{\pi}{4}(1-4\mu)-\pi\mu^2\), we can trivially pack all the circles in the bin using $\mathtt{greedyNFDR}$ and the theorem holds trivially since \(1 \geq  \frac{\pi}{4}(1-4\mu)-\pi\mu^2\) . Otherwise note that if $a_i$ denotes the area of the $i^{th}$ circle in $S$, \[\sum_{i=1}^{s}a_i \geq  \frac{\pi}{4}(1-4\mu)-\pi\mu^2\] Also since the total area of all the circles is less than 1 \[\sum_{i=s+1}^{n}a_i \leq  1-(\frac{\pi}{4}(1-4\mu)-\pi\mu^2)\]
	Also all the circles in \(S_{\text{packed}}\) have radius \(\leq r_{s}\) and among all the possible sets of \(S_{\text{packed}}\), $S$ will be minimum when all the circles in \(S_{\text{packed}}\) have radius \(r_{s}\). Hence we can bound s as \[s \geq \frac{\frac{\pi}{4}(1-4\mu)-\pi\mu^2}{\pi r_{\text{s}}^2}\]
	Also all the circles in \(S_{\text{unpacked}}\) have radius \(\geq r_{s}\) and among all the possible sets of \(S_{\text{unpacked}}\), the cardinality of the set \(S_{\text{unpacked}}\) will be maximum when all the circles in \(S_{\text{unpacked}}\) will have radius \(r_{s}\). Hence we can bound the cardinality of the set \(S_{\text{unpacked}}\) as \[n-s \leq \frac{1-(\frac{\pi}{4}(1-4\mu)-\pi\mu^2)}{\pi r_{\text{s}}^2}\] where $n$ is the total number of circles in $S$. Therefore the minimum value of \(\frac{s}{n}\) can be bound as
	\begin{align*}
		\frac{s}{n} \geq \frac{\frac{\frac{\pi}{4}(1-4\mu)-\pi\mu^2)}{\pi r_{\text{s}}^2}}{\frac{(\frac{\pi}{4}(1-4\mu)-\pi\mu^2)}{\pi r_{\text{s}}^2} + \frac{1-(\frac{\pi}{4}(1-4\mu)-\pi\mu^2)}{\pi r_{\text{s}}^2}} \\
		\Rightarrow \frac{s}{n} \geq \frac{\pi}{4}(1-4\mu)-\pi\mu^2
	\end{align*}
	Hence we will always be able to pack \(\frac{\pi}{4}(1-4\mu)-\pi\mu^2\) times the optimal total number of circles using $\mathtt{greedyNFDR}$.
\end{proof}







Let $\OPT$ be the optimal packing for $\mathsf{CSK}$ and $\mathcal{C}_{\OPT}$ be the set of circles in $\OPT$. 
We first partition set $\mathcal{C}$ of circles into three groups based on the size of their radii and an input parameter $\eps>0$ called small, medium, and large. We also assume \(\eps \leq 0.1\) and our algorithm successfully provides a valid packing for these bound on \(\eps\) We choose the bounds on radii for partitioning such that the medium circles have a total profit of at most $\eps\cdot w(\OPT)$ and hence ignore the medium circles from now on, losing a small amount of profit.

We then pack the large circles from $\mathcal{C}_{\OPT}$ in our unit bin using an approximation scheme and call the packing $P^+$. Depending on the number of large circles compared to number of small circles, we choose to pack different set of circles in our final packing. If there are not too many small circles in $\mathcal{C}$, we can simply pack them in the pocket created by three or more touching large circles in $P^+$ and pack the small circles inside the pocket using the algorithm mentioned in \cite{Fekete2019PackingDI} for packing disks into disks to further get packing  \(P^*\) from \(P^+\). If there are a large number of small circles, we can kill off all the large circles, losing only a small amount of profit and approximate pack only the small circles in \(\mathcal{C}\) into the unit bin to get our desired packing \(P^*\).
When there are only a small number of circles in $\mathcal{C}_{\OPT}$, we can simply pack using brute force using lemma \ref{threepack}. We prove that this scheme results in a worst case approximation ratio of $5/3$.
\subsubsection{Partitioning the set of circles} \label{partiotion section}
We partition our set $\mathcal{C}$ using ideas from section \ref{medium}. We select the function according to our needs, ensuring a significant gap in the radii of large and small circles. This choice is crucial for establishing various structural properties.\\
Define $\rhoi{0} = \frac{1}{2}$, and $\rhoi{k} = \frac{1}{2}\times\rhoi{k-1}^2\eps$ for all integers $k \geqslant 1$. Then,

\begin{equation}
	\label{rho_k_new}
	\rhoi{k} = \frac{\eps^{2^{k}-1}}{{2^{2^{k+1}-1}}}
\end{equation}

For each integer $k \geqslant 1$ we define the following sets of circles:
\begin{align*}
	S_k = \{c_i \in S \mid r_{i} \in (\rho_{k},\rho_{k-1}]\}
\end{align*}

 We then remove medium circles from further consideration and lose at most $\eps$ fraction of the total number of circles. In the next sections, we show how to modify $\OPT$ to produce a packing of circles in \(\mathcal{C}_{L}^*\)to a packing $P^+$ with a very regular structure. We will further extend \(P^+\) to a packing \(P^*\) with including \(\mathcal{C}_{L}*\) and \(\mathcal{C}_{S}^*\)

To describe the construction of $P^*$, we need to consider two separate cases: (i) when $\mathcal{C}_{L}^* = \varnothing$, and (ii) when $\mathcal{C}_{L}^* \neq \varnothing$
\subsubsection{Packing the Big Circles} \label{Big_Circle_Pack}

When $\mathcal{C}_{L}^* = \varnothing$,we first remove all the medium circles in $\OPT$ to get a set of small circles $\mathcal{C}_{S}^*$ of profit at least $(1-\eps)w(\OPT)$ in which all remaining circles have radius at most $\rho_{\tau} \leq \frac{\eps}{8}$, as $\tau \geq 1$. We will pack these circles using the greedyNFDR as described in lemma \ref{greedyNFDR_lemma}  for unit weight circles. Using this strategy we will be able to pack at least \(\frac{\pi}{4}(1-4\rho_{\tau})-\pi\rho_{\tau}^2\) times the total number of small circles in our optimal solution. Since \(\rho_{\tau} \leq \frac{\eps}{8}\).We will always be able to pack more than \(\frac{3}{5}\) times the total number of small circles in optimal solutionfor $\eps \leq 0.1$.

Now we deal the case when then number of circles in \(\mathcal{C}_{L}^*\) is non-zero. If the number of large circles in \(\OPT\) is less than 6 we proceed as follows. We first remove all the medium circles $\mathcal{C}_M ^*$ in \(\OPT\) from the packing. We also remove all the small circles $\mathcal{C}_S ^*$ temporarily for now. We will add them back later. Now we are only left with large circles in the bin. Then we can modify their packing using Lemma \ref{threepack} and pack 1 large circle when there is 1 large circle in \(\OPT\), 2 large circles when there is 2 large circles in \(\OPT\) or pack 3 large circles when there is either 3, 4, or 5 large circles in \(P\). 

\begin{figure}[ht]
	\begin{center}
			\includegraphics[width=6cm]{Images/4 by 3 apx figure.pdf}
		\caption{\(1\times 1\) bin with \(1\times\rho_{\tau-1}\) strips along the four sides to modify packing of large circles}
		\label{fig:4-by-3-apx-img}
		\end{center}

\end{figure}

Now we look at the case when, the number of large circles in \(\OPT\) is more than 5. Here is the scheme of things we follow to arrive at the structure we want. We begin with an optimal packing \(\OPT\) in the square bin \(ABCD\) as shown in figure \ref{fig:4-by-3-apx-img}. We first remove all the medium circles $\mathcal{C}_M ^*$ in \(\OPT\) from the packing. We also remove all the small circles temporarily for now. We will add them back later. Now we are only left with only circles in \(\mathcal{C}_{L} ^*\) in the bin. If the number of large circles is \(6\) or more circles.  We define the following cuts on the packing of \(\mathcal{C}_{L}^*\): \(\ell_1\) representing the line \(EG\), \(\ell_2\) representing the line \(GH\), \(\ell_3\) representing the line \(FH\), and \(\ell_4\) representing the line \(EF\). These cuts are made at a distance of \(\rho_{\tau-1}\) from the sides of the bin. Recall that all our large circles have a radius \(\geq \rho_{\tau-1}\). Also we assume that there exists no circle with radius \(\geq \frac{1}{2}-\rho_{\tau-1}\) that is no circle intersects two diametrically opposite strips. We will deal this case separately when there exists a circle with radius \(\geq \frac{1}{2}-\rho_{\tau-1}\). These cuts will generate four rectangular regions, \(R_1,R_2,R_3,\) and \(R_4.\) The rectangular regions include the shaded corners as well. The grey shaded corners are squares of dimension \(\rho_{\tau-1}\times\rho_{\tau-1}.\) These will be essential, as we prove important structural lemmas involving these four regions.

\begin{lemma}
	\label{only4-circles}
	At most one large circle can intersect each of the grey regions. In other words, at most 4 large circles can intersect the regions shaded grey. 
\end{lemma}
\begin{proof}
	To prove the claim, we will analyze the grey region on bottom left between point C,G and same arguments can be used for the other grey squares as well.
	For a large circle to intersect the grey squares, its center must lie in a `feasible region'. For a (large) circle of radius \(\rho_{\tau-1}\) and the region enclosed between point \(G,C\) the feasible region would be a quarter circle centered at \(G\) of radius \(\rho_{\tau-1}\) since if the center lies beyond a distance of \(\rho_{\tau-1}\) from \(G\) then, it's not possible for it to intersect the grey square. 
	
	Consider the feasible regions for the centers of two circles of radius \(r_1,r_2\geqslant\rho_{\tau-1}\), the feasible region would be quarter of a circle. For example, consider the circle with radius \(r_1\) and focus on it's center. One case where the circle intersects the maximum of the grey square is when it's center lies at the point \((r_1,r_1)\). The other extreme case will be when the circle intersects just \(G\) as in Fig. \ref{fig:4-by-3-apx-img}. And rest of the conditions will be imposed by the fact that the circle cannot go out of the bin. So, this will end up tracing a quarter circle where the arc will be defined by the equation \((x-\rho_{\tau-1})^2+(y-\rho_{\tau-1})^2=r_1^2\), and the lines \(x=r_1\), \(y=r_1\). The intersection of these will trace out the quarter circle. 
	
	Let the feasible region of the center of the circle with radius \(r_1\) be \(FR_1\), for \(r_2\) be \(FR_2\). Observe that the center of the feasible regions will always lie on the line \(y=x\) because of the above construction. To have a non-intersecting configuration of circles there needs to be at least a distance of \(r_1+r_2\) between their centers. When \(FR_1\cap FR_2 = \varnothing\), we claim that the maximum distance between any two points in \(FR_1\) and \(FR_2\) is less than the required \(r_1+r_2\) and thus, we cannot have a non intersecting configuration of two circles with both of them intersecting the grey square. From preliminary observation we can see that the two points furthest apart from each other must lie on the part defined by straight lines for \(FR_1\) and the arc for \(FR_2.\) 
	
	\begin{figure}[ht]
		\centering
		\includegraphics{Images/large_circle_corner_lemma.pdf}
		\caption{(a) The orange region highlights the feasible region for the dashed circle. (b) An illustrative example of the points and lines required for the proof of claim.}
		\label{fig:enter-label}
	\end{figure}
	\begin{claim}
		The center of \(FR_1\) and the point where \(y=x\) intersects \(FR_2\) are the two points which are furthest apart from each other.
	\end{claim}
	\begin{claimproof}
		Let, \(X\) be the center of \(FR_1\) and $Y$ be the point where \(y=x\) intersects the arc of \(FR_2.\) Now consider any point \(X'\) either on \(x=r_1\) or \(y=r_1\) on \(FR_1\) and \(Y'\) on the arc of \(FR_2.\) The shortest distance between both of them will be the straight line joining them. Now, join \(X\) and \(Y\) along a straight line and let it intersect \(FR_1\) at \(P\) and \(FR_2\) at \(Q\), now observe that, 
		\begin{align*}
		X'Y' &\leqslant X'P+PQ+Y'Q \\
		&\leqslant XP+PQ+YQ \\
		&= XY.
		\end{align*}
		Thus giving us that the longest distance between any two points on \(FR_1\) and \(FR_2\) when \(FR_1\cap FR_2=\varnothing\) is \(XY.\) 
	\end{claimproof}
	Now using standard cartesian coordinate system, we can figure out that the coordinates of \(X\) are \((r_1,r_1)\) and the coordinates of \(Y\) are \((r_2/\sqrt{2}+\rho_{\tau-1},r_2/\sqrt{2}+\rho_{\tau-1})\) due to the construction of \(FR_2.\) Now, applying the distance formula we prove that \(XY<r_1+r_2\) always. Let \(d\) be the distance/length of \(XY\), then
	
	\begin{align*}
	d^2 &= \Le(\frac{r_2}{\sqrt{2}}+\rho_{\tau-1}-r_1\Ri)^2+\Le(\frac{r_2}{\sqrt{2}}+\rho_{\tau-1}-r_1\Ri)^2 \\
	&\approx \Le(\frac{r_2}{\sqrt{2}}-r_1\Ri)^2+\Le(\frac{r_2}{\sqrt{2}}-r_1\Ri)^2 \\
	&= 2\Le(r_1^2+\frac{r_2^2}{2}-r_1r_2\sqrt{2}\Ri) = r_1^2 + (r_1^2+r_2^2-2\sqrt{2}r_1r_2)\\
	&\leqslant r_1^2 + (r_1^2+r_2^2 - 2r_1r_2) \\
	&= r_1^2 + (r_2-r_1)^2 \\
	&\leqslant r_1^2+r_2^2 \\
	&< r_1^2+r_2^2+2r_1r_2 = (r_1+r_2)^2
	\end{align*}{\tiny }
	Thus, we have that \(d\leqslant(r_1+r_2).\) Now the case then \(FR_1\subset FR_2\) is trivial to observe. Since one feasible region is contained in another we cannot have any selection of two points such that their distance is greater than \(r_1+r_2.\) Similarly for the case when \(FR_1\cap FR_2 \neq \varnothing\) observe that the the distance between the previously defined points \(X\) and \(Y\) decrease because of the two feasible regions intersecting each other. So naturally, the length of \(XY\) decreases as well, and since in the previous case we saw that \(d< r_1+r_2,\) this will apply to this case as well. Hence, we have that at most one large circle can intersect the grey squares.
\end{proof}
We call the circles which intersect at least two strips, or equivalently the grey region as shown in figure \ref{fig:4-by-3-apx-img}, \textit{corner circles}.
\begin{lemma}
	\label{delete-one-repack}
	{If there are many circles along with the corner circles which intersect two adjacent strips (\(R_i\) and \(R_{i-1}\) or \(R_{i+1}\)) we can always remove the largest circle in \(\mathcal{C}_{L}^*\) which intersect the strips and pack the circles which intersect two strips simultaneously into the space occupied by the removed circle.}
\end{lemma}
\begin{proof}
	Without loss of generality, we will consider the case of the strips \(R_1\) and \(R_4\). In order to prove this lemma, first let us consider the ordering of the cirlces which intersect two adjacent strips \(R_1\) and \(R_4\) as \(\mathcal{C}_{\text{intersect}}=\{C_1,...,C_m\}\) in the increasing order of their corresponding centers' distance from the point \(A\). Let us also denote the radius of circle \(c_i\) with \(r_i\). In order to prove our lemma we will find the lower bound for \(\frac{r_i}{r_{i-1}}\). First we observe that all the circles in \(\mathcal{C}_{\text{intersect}}\) have radius \(\geq \rho_{\tau-1}\). For a particular fixed circle \(C_i\) with radius \(r_i\), the radius of the \(i-1\)-th circle \(C_{i-1}\) will be maximum when the \(i\)-th circle and \(i-1\)-th circle touch two opposite boundaries of the bin and only touch the other side strip as shown in Figure \ref{fig:enter-label}.
	\begin{figure}[H]
		\centering
		\includegraphics[width=0.5\textwidth]{Images/consequitive_circle_in_square} % Scale image to the width of the text
		\caption{Two consecutive circles intersecting two adjacent strips R1 and R4}
		\label{fig:enter-label}
	\end{figure}
	Notice that in this case, we have \(O_nO_{n-1}=r_i+r_{i-1}\), \(O_nE=r_i-r_{i-1}-\rho_{\tau-1}\) and \(O_{n-1}E=r_i\). Applying Pythagoras theorem on triangle \(O_nO_{n-1}E\), we have

\begin{gather*}
	(r_i+r_{i-1})^2 = (r_i-r_{i-1}-\rho_{\tau-1})^2 + (r_i)^2 \\
	r_i^2 - 2\rho_{\tau-1}r_i + 2\rho_{\tau-1}r_{i-1} - 4r_ir_{i-1} + \rho_{\tau-1}^2 = 0
\end{gather*}
 For the ratio \(\frac{r_i}{r_{i-1}}\), consider two boundary cases. First, we consider the case when \(r_{i-1}=\rho_{\tau-1}\), that is \(r_{i-1}\) reaches it's minimum possible value. In this case we get, \(r_i=(3+\sqrt{6})\rho_{\tau-1}\). In this case \(\frac{r_i}{r_{i-1}}=3+\sqrt{6}>4\). Second we consider another boundary case, that is \(r_i=\frac{1}{2}\). In this case \(r_{i-1}=\frac{(\frac{1}{2}-\eps)^2}{2(1-\eps)}\). So in this case, we have \(\frac{r_i}{r_{i-1}}=\frac{(1-\eps)}{(\frac{1}{2}-\eps)^2}\geq 4\). It follows that \(\frac{r_i}{r_{i-1}}\geq 4\),we first note that \(r_i \leq r_n (\frac{1}{4})^{m-i}\) and we can make the following claim about the sum of area of circles from \(1 \text{ to } m-1\) in comparison to the area of the \(m\)-th circle. Denote the area of the \(i\)-th circle by \(A_i\). It follows that
 
\begin{center}
	\(\sum_{i=1}^{m-1} A_i \leq \sum_{i=1}^{m-1} \pi \left(r_m\left(\frac{1}{4}\right)^{m-i}\right)^2 = \sum_{i=1}^{m-1} \pi r_m^2 \left(\frac{1}{16}\right)^i < \frac{\pi r_m^2}{15} = \frac{A_m}{15}\)
\end{center}
	Now consider an inscribed axis parallel square inside the circle with radius $r_m$. This has an area of $2 r_m^2$. Using the Splitpacking algorithm from \cite{10.1007/978-3-540-39658-1_20}, we know that since the total area of the circles with radii $r_1,..., r_{m-1}$ is at most $0.53\cdot2r_m^2$, we can pack them inside the inscribed square in polynomial time.
\end{proof}
Now let us handle the case when there exists one huge circle in \(\mathcal{C}_{L}^*\) with a diameter greater than or equal to \(1-2\rhoi{\tau-1}\). Getting a partition in this case using our cuts is difficult because the \textit{huge} circle will intersect all of the \(R_i\)'s. But, in this case we can just delete the large circle from our packing \(P\) altogether. Notice that the area remaining after deleting the huge circle is atmost \(1-\frac{\pi}{4}(1-2\rhoi{\tau-1})^2\). Since \(\tau \geq 2\), we have \(\rhoi{\tau-1}\leq\frac{\eps}{8}\)\(\) and so we can bound the area of the remaining cirlces as \(1-\frac{\pi}{4}(1-2\rhoi{\tau-1})^2 \leq 1-\frac{\pi}{4}(1-\frac{2\eps}{8})^2 \leqslant 0.53 \). Now, using \cite{SplitPack} which claims that ``any set of circles with a combined area of up to 53.90\% of the square’s area can be packed" we can generate the approximate packing \(P^*\) which our algorithm will return. This \(P^*\) will have a profit of \(w(\OPT)-1.\) 

Now we consider the case when there is no large circle with diameter greater than or equal to \(1-2\rhoi{\tau-1}\).  Recall the rectangular strips \(R_i\)'s generated before. We now define \(C_1,C_2,C_3\) and \(C_4\) to be the set of disks in \(\mathcal{C}_{L}^*\) which only intersect only one of the above rectangular strips. If a circle intersects only one of \(R_i\)'s then it's included in the set \(C_{i}\). If a disk intersects both \(R_1\) and \(R_2\) then it's not a part of \(C_1\cup C_2\cup C_3\cup C_4.\) We will give a scheme to get rid of all such disks by removing at most one circle from each of the corner. The above creates a partition which will help in the analysis. Put the disks not in any of the \(C_i\)'s above in a set \(C_X.\) 

We do the following modification to the packing of large circles
\begin{enumerate}
	\item If we observe multiple disks which intersect or touch two adjacent rectangular strips then we use Lemma \ref{delete-one-repack} to handle this case and obtain the complete partition by removing the largest of such intersecting disks. The circles now do not intersect two adjacent strips anymore and now they are contained in \(C_X\). Notice that in this case, we get rid of the problematic case of circles intersecting multiple strips by removing at most one circle from each of the corner.\label{step3}
	\item Otherwise if we observe that if there is only a single disk which intersect or touch two adjacent rectangular strips or the shaded grey region then we just remove the circle and obtain the complete partition. In this case also we get rid of the problematic case of circles intersecting multiple strips by removing at most one circle from each of the corner.\label{step4}
	\item Partition the disks into sets \(C_1,C_2,C_3,C_4,\) and \(C_X.\) Where each set \(C_i\) contains those disks which only intersect \(R_i.\) \(C_X\) contains those which don't belong to any of the other \(C_i\)'s.
	\item Among \(C_1,C_2,C_3,C_4\) we remove the `cheapest' set of disks and also remove the \(1\times\rhoi{\tau-1}\)-size strip corresponding to that set, which in this case means removing the set with the least number of disks. We get a packing of the other 3 sets along with the set \(C_X\) in a bin of size \(1\times(1-\rhoi{\tau-1})\). Now we add back the circles removed in step \ref{step3} and set \ref{step4} to at least two of the corner of the \(1\times(1-\rhoi{\tau-1})\) sized bin.
\end{enumerate}

\begin{lemma}
	\label{rationalization-1-eps}
	We can rationalize the large circles' coordinates in the cuts generated \(1\times(1-\rhoi{\tau-1})\) bin by augmenting the bin by an \(\rhoi{\tau-1}\) factor. That is, we can augment the circles to have rational centers in a \(1\times1\) bin.
\end{lemma}
\begin{proof}
	We call the  \(1\times(1-\rhoi{\tau-1})\) bin as R.
	Let us begin by bounding \(n\), i.e., the number of large circles possible. To do this we make the observation that the total area of the large circles cannot exceed the area of \(R\). So we have \(n\pi(\rhoi{\tau-1})^2<1-\rhoi{\tau-1}\). This gives us, \(n<({1-\rhoi{\tau-1}})/{\pi\rhoi{\tau-1}^2}.\)  
	
	Now, we focus on rationalizing the \(x\)-coordinates. Number the circles in increasing value of $x$-coordinate from left to right. If two circles have the same $x$-coordinate, then order the one with the lower $y$-coordinate before the one with the higher $y$-coordinate. Let the $x$-coordinates of the $n$ circles in $P$ be $x_1,x_2,\ldots,x_n$. We propose the following (re-)packing scheme. For circle \(i\in P\) shift it to the right by \(\Delta x_i\) amount such that the shifts themselves follow the order \(\Delta x_1 < \Delta x_2 < \cdots <\Delta x_n\). Observe that this shifting scheme preserves the non-intersecting nature of the packing. 
	
	Superpose a semi-grid of side length \((\rhoi{\tau-1})^k\) on the bin, i.e., we superpose a grid (in which distance between two vertical lines is \((\rhoi{\tau-1})^k\) on the bin we have) where $k$ is a given integer. Observe that any line segment of length \((\rhoi{\tau-1})^k\) will have at least one integral multiple of \((\rhoi{\tau-1})^k\),  and hence we can get a suitable \(\Delta x_1 < \rhoi{\tau-1}^k\) such that the first circles aligns itself up on a grid line. We can similarly also find a \(\Delta x_2 < (\Delta x_1 + \rhoi{\tau-1}^k)+2\rhoi{\tau-1}^k\) where the \(2\rhoi{\tau-1}^k\) term is added to be used later as extra space. Note that the extra space we added leads to the property that $x_i- x_{i-1} \geqslant 2\rhoi{\tau-1}^k$ for $i=2,3,...,n$. Extending this for the \(n^{th}\) circle, we get \(\Delta x_i<(3i-2)\rhoi{\tau-1}^k.\) The only constraint is that the total displacement of the circles at the end should be at most \(\rhoi{\tau-1}\), so we get the following inequality as a sufficient condition for us to find a integral $x$-coordinate for every circle using the shifting scheme described above-  
	\[\Delta x_n<\rhoi{\tau-1}\Rightarrow (3n-2)(\rhoi{\tau-1})^k<\rhoi{\tau-1} \Rightarrow n < \frac{2}{3}+\frac{1}{3(\rhoi{\tau-1})^{k-1}}.\] Notice that this condition is satisfied from the area bound on $n$ at the beginning of the section for all $k \geq 3$ and a $\rhoi{\tau-1} < 0.5$, which is guaranteed as we have a bound on $\eps$ later on in the paper. Hence we can always shift the x-coordinates of the circles to fit themselves on a $(\rhoi{\tau-1})^k$ grid for $k \geq 3$.
	
	Intuitively, moving circles to the right in the $x$-direction will free up some space in the $y$-direction for the circles to move. Let us assume that this space from the $x$-movement above allows us to fit everything to an $\rhoi{\tau-1}^{\ell}$-grid in the $y$-direction (i.e., the grid-lines are horizontal now) with $\ell\geqslant k$ from above. We are now superposing a finer grid on the bin than the one we superposed above. 
	
	\begin{figure}[ht!]
		\centering
		\includegraphics[width=7cm]{Images/rational.png}
		\caption{The \(i^{\text{th}}\) circle and it's neighbors.}
		\label{fig:circles_rational}
	\end{figure}
	
	Now, consider the vertical movement to find integral coordinates for the $i^{\text{th}}$ circle.  Assume that it has $N$ ``neighbors" in the packing $P$. Neighbors are defined as the circles with an index larger than $i$ that disallow movement of the $i^{\text{th}}$ circle in the vertical $y$ direction by $\rhoi{\tau-1}^{\ell}$ (see Fig. \ref{fig:circles_rational}). The $i^{th}$ circle and its neighbors have the $y$-coordinates $y_i$ and $Y_1, Y_2, \cdots Y_N$. Let our rearrangement scheme move each of the circles by $\Delta y_i$ and $\Delta Y_1, \Delta Y_2, \cdots, \Delta Y_N$, respectively.
	The $i^{\text{th}}$ circle can have a maximum radius of $\frac{1}{2}$ as it is packed inside a $1\times 1$ square. The $x$-coordinate of the center of its $N$ neighbors have to be to the right of the $x$-coordinate of the $i^{\text{th}}$ circle. Because these are the only circles whose movement can free up space for the \(i^{\text{th}}\) circle to move in the \(y\)-direction. Since each of the $N$ neighbors have a radius of at least $\rhoi{\tau-1}$, we get that $N<\frac{2}{\rhoi{\tau-1}}$ from perimeter equations for $\rhoi{\tau-1}<0.5$, which is guaranteed by the bound on $\eps$ later.
	
	Due to the additional `\(2\rhoi{\tau-1}^k\)' factor which we added above in the rationalising scheme for the $x$-coordinates, we can claim that for each neighbor $j$ of the \(i^{\text{th}}\) circle we have $X_j- x_i \geq 2 (\rhoi{\tau-1})^k$. Since the circles were tightly packed before and now have an extra space of $X_j- x_i \geq 2 (\rhoi{\tau-1})^k$, using the expansion of cosine for small angles, we get that
	% \textcolor{red}{Using simple trigonometric arguments} \textcolor{blue}{[P: please add and and all arguments and calculations explicitly]}, this leads to 
	the space for movement in the y-direction is  such that $|\Delta Y_j|+ |\Delta y_i| \geq (\rhoi{\tau-1})^{2k}$.
		
	% After the circle has moved along the \(x\)-direction, recall the fact that the shortest distance between two circles is \(C_1C_2-r_1-r_2\), where \(C_1C_2\) is the distance between the centers of the two circles and \(r_1,r_2\) are their respective radii. So, after joining both the centers using a line segment observe that the `allowed' \(y\)-axis movement will be the vertical projection of the ``shortest distance" as highlighted by the small black triangle in Figure \ref{fig:tan_argument}. Consider the triangle formed by the old center \((C_1^o)\), the new center \(C_2^n\) (of the small circle) and the center of the big circle \((C)\). Observe that, \(C_1^oC=r_1+r_2\) where \(r_1\) is the radius of the large circle and \(r_2\) is the radius of the small circle and \(C_1^oC_1^n\geqslant 2\rhoi{\tau-1}^k\). Using this information, and applying the sine and cosine rules repeatedly, we can figure out the angle \(\angle C_1^oCC_1^n\) and length \(CC_1^n\). Using that, we can calculate the vertical projection of the smallest distance between the circles, which comes out to be greater than \(2\rhoi{\tau-1}^{2k}.\) 
	Now, we have to consider the vertical movement of each of the \(N\) neighbors. If $l \geq 2k+1$, then we have at least $\frac{2}{\rhoi{\tau-1}}$ integral points in the vertical free space ($2(\rhoi{\tau-1})^k$) for the $i^{th}$ circle. So we can find a $\Delta y_i$ such that $y_i$ lands on an integral coordinate. We do this for each circle $i$. In addition, we are guaranteed that for movements in the $N$ neighbors in further steps, we are sure to find a free integral y-coordinate as $N<\frac{2}{\rhoi{\tau-1}}$.
	
	% Since we have generated a `vertical free space' of \(2\rhoi{\tau-1}^{2k}\), so in a \(\rhoi{\tau-1}^{2k+1}\) grid, we will have \(\frac{2\rhoi{\tau-1}^{2k}}{\rhoi{\tau-1}^{2k+1}}=\frac{2}{\rhoi{\tau-1}}\) integral grid points. Now, we know \(N<\frac{2}{\rhoi{\tau-1}}\), so we can find at least one integral grid point for the \(N+1\) (`+1' because we add the `\(i^{\text{th}}\)' circle itself as well) circles under consideration. Hence, we observe that any grid of width \(\ell\geqslant 2k+1\) will work.
	Now, for concrete values we substitute \(k=3\) which gives us that everything can be fit into a \(\rhoi{\tau-1}^{2\cdot 3+1} grid.\) These values can be optimised a bit but we do not care too much about that. We can see that everything can be fit into an $\rhoi{\tau-1}^7$-grid after augmenting one of the sides of the square.
\end{proof}
% \subsection{Packing the big circles onto the grid}
%Now after rationalisation, we pack the big circles onto the grid in constant time. To prove that we can do so in constant time, we first note that the number of big circles is bounded by a constant as each big circle has a radius of at least $\eps$ and the total area of the bin is $1$. Now, there are again a constant number of subsets possible of the set of all big circles. Using rationalisation in coordinates in the augmented bin, we achieve constant number of possible packings for each subset of the big circle. Henceforth, we can find a rationalised packing of the big circles with maximum profit in constant time and proceed with it for the rest of the procedure. %
We had a packing of a subset of \(\mathcal{C}_{L}^*\) in a bin of size  \(1\times(1-\rho_{\tau-1})\). We will now augment the bin to have dimension \(1\times1\) with all the circles having rational coordinates to their corresponding centers using lemma \ref{rationalization-1-eps}. We call this packing \(P^+\).
The final structural claim we make about the weight of \(P^+\) is that the modified packing is guaranteed to have weight 
	\[
	w(P^+)= 
	\begin{cases}
	\lvert \mathcal{C}_{L}^* \rvert, & \lvert \mathcal{C}_{L}^* \rvert\leq 3 \\
	3, & 4 \leq \lvert \mathcal{C}_{L}^* \rvert \leq 5 \\
	\lceil\frac{3}{4}\cdot\lvert \mathcal{C}_{L}^* \rvert\rceil-1 & 6 \leq \lvert \mathcal{C}_{L}^* \rvert
	\end{cases}
	\]
    In the case when the number of large circles is $<6$, we use lemma \ref{threepack} , and the profit of the packing is straightforward from the packing strategy. In the other case, we note that,
	there can be a maximum of 4 circles removed from each of the corners during generating the partitioning, we are left with at least \(\lvert \mathcal{C}_{L}^* \rvert-4\) disks. Now, we remove the set \(C_i\) \(i\in\{1,2,3,4\}\) which has the least number of disks (which translates to the cheapest set among all \(C_i\)'s). This will result in loss of atmost \(\left\lfloor\frac{\lvert \mathcal{C}_{L}^* \rvert-4}{4}\right\rfloor\) profit. After the removal we add atleast two of the circles which we have earlier removed during the partitioning in their original positions and so the final number of large circles in \(P^+\) is atleast \[\lvert \mathcal{C}_{L}^* \rvert-4+2-\left\lfloor\frac{\lvert \mathcal{C}_{L}^* \rvert-4}{4}\right\rfloor = \left\lceil\frac{3}{4}\cdot\lvert \mathcal{C}_{L}^* \rvert\right\rceil-1\]
\subsubsection{Packing the small circles} \label{Small-Circle-Pack}
Now we will add back the small circles in \(P^+\) to get the final packing structure \(P^*\). Let us denote the total area of small circles in \(\mathcal{C}_{S}^*\) as \(A_{\text{small}}\) and the total area of large circles in \(\mathcal{C}_{L}^*\) as \(A_{\text{large}}\).
% Consider two separate cases as follows.

\textbf{Case - I : } \(A_{\text{small}} \leq A_{\text{large}}\times \frac{\rho_{\tau-1}^2}{30}\)

When the combined area of small circles in \(\mathcal{C}_{S}^*\) is very small as compared to the total area of large circles, we can pack all the small circles in the pocket created by three or more touching large circles in \(\mathcal{C}_{L}^*\) or pack them by removing at most one large circle.

First, consider the case when the number of large circles in \(\mathcal{C}_{L}^*\) is 1. In this case, the large circle will have a radius \(\leq \frac{1}{2}\). If our packing has a large circle of radius at most \(\frac{1}{2}\), then we can have a imaginary circle of radius at least\(\frac{\sqrt{2}-1}{2(\sqrt{2}+1)}\) touching two sides of the bin at one of the corners and not intersecting the large circle. We know that the total area of small circles is at most \(\pi (\frac{1}{2})^2 \cdot \dfrac{\frac{1}{4}}{30}=\frac{\pi}{480}\). The imaginary corner circle has area at least \(\pi (\frac{\sqrt{2}-1}{2(\sqrt{2}+1)})^2\). Using the algorithm in \cite{Fekete2019PackingDI} for packing circles into circles, we can pack all the small circles in the imaginary circles since \(\frac{\pi}{480}\leq \frac{1}{2}\cdot\pi(\frac{\sqrt{2}-1}{2(\sqrt{2}+1)})^2\) and we get packing for all the small circles in \(\mathcal{C}_{S}^*\) along with the large circle in \(\mathcal{C}_{L}^*\).

For the case when number of large circles in \(\mathcal{C}_{L}^*\) is 2. We pack the small circles using different approaches depending upon the number of small circles. If the number of small circles in \(\leq 3\). We have at most 5 circles and we can pack them in the bin using lemma \ref{threepack} and always pack 3 out of at most 5 circles.

Other wise in this scenario we choose the biggest of the two large circles that is already packed in our bin. Note that this circle has radius at least \(\rho_{\tau-1}\). Consider the square of maximum area that can be inscribed this circle and has sides parallel to that of the bin. We replace the circle with this square and name it as \(S\). This square has side length at least \(\rho_{\tau-1} \times \sqrt{2}\). Also note that \(A_{\text{large}} \leq 1\)  implies \(A_{\text{small}} \leq \frac{\rho_{\tau-1}^2}{4}\) and all the small circles have radius \(\leq \rho_{\tau}\). We pack all the small circles in \(S\) using NFDR. For circles with radius less than \(\rho_{\tau}\), we can pack either all the circles or circles with total area at least \(\frac{\pi}{4}(2\rho_{\tau-1}^2-4\sqrt{2}\rho_{\tau-1}\rho_{\tau})\)
in a square with side length \(\rho_{\tau-1}\times\sqrt{2}\). Note that \(\rho_{\tau} = \frac{1}{2} \times \rho_{\tau-1}^2\eps\). 
Hence we can see
\begin{align*}
\frac{\pi}{4}(2\rho_{\tau-1}^2-4\sqrt{2}\rho_{\tau-1}\rho_{\tau})=\frac{\pi}{4}(2\rho_{\tau-1}^2-2\sqrt{2}\rho_{\tau-1}^3\eps) \geq \frac{\rho_{\tau-1}^2}{30}
\end{align*}
 Hence, we can pack all the small circle in \(P\) by replacing one big circle from our bin.

For the case when the number of large circles in \(\mathcal{C}_{L}^*\) is \(\geq 3\), we will pack all the small circles in \(\mathcal{C}_{S}^*\) in pocket created by three or more touching large circles. In the packing \(P^+\) of large circles in \(\mathcal{C}_{L}^*\), all the circles have radius \(\geq \rho_{\tau-1}\). In this packing of the large
we can find a pocket created by three or more touching large circles and embed an imaginary circle in it . In order to provide a feasible packing of small circles, we need to find lower bound for the radius of the imaginary circle in the pocket. We can note that the imaginary circle in the pocket will have the least radius when it is created by three mutually touching circles of radius \(\rho_{\tau-1}\).
%\begin{center}
%	\begin{tikzpicture}
%	% Define the radius of the large circles
%	\def\Radius{2cm}
%	% Calculate the radius of the small circle
%	\def\smallRadius{(\Radius*(2-sqrt(3))) / sqrt(3)}
%	
%	% Define coordinates for the centers of the large circles
%	\coordinate (X) at (0,0);
%	\coordinate (Y) at ($(X) + (60:2*\Radius)$);
%	\coordinate (Z) at ($(X) + (0:2*\Radius)$);
%	
%	% Draw the large circles and label their centers
%	\draw (X) circle (\Radius);
%	\draw (Y) circle (\Radius);
%	\draw (Z) circle (\Radius);
%	\node at (X) [below] {X};
%	\node at (Y) [above] {Y};
%	\node at (Z) [below] {Z};
%	
%	% Calculate the center of the small circle (centroid of the triangle)
%	\coordinate (O) at (barycentric cs:X=1,Y=1,Z=1);
%	
%	% Draw the small circle and label its center
%	\draw (O) circle (\smallRadius);
%	\node at (O) [below] {O};
%	\end{tikzpicture}
%\end{center}
\begin{figure}[ht]
	\begin{center}
		\includegraphics[width=7cm]{Images/3-circles-touching.pdf}
		\caption{Packing small circles in the \textit{pockets} of the large circle packing}
		\label{fig:pocket}
	\end{center}
	
\end{figure}
If the circles with center at \(X,Y,Z\) each have radius \(\rho_{\tau-1}\). Then the circle with center O in the pocket created by the three big circles will have radius \(\rho_{\tau-1}\times\frac{2-\sqrt{3}}{\sqrt{3}}\).
This is the least possible radius of a circle in a pocket created by three or more circles. Note that in this case the total area of small circles is \(A_{\text{small}} \leq A_{\text{large}}\times \frac{\rho_{\tau-1}^2}{30}\leq\frac{\rho_{\tau-1}^2}{30}\). Using the algorithm in \cite{Fekete2019PackingDI} for packing disks into disks, we can pack all the small circles in the imaginary disk in the pocket since \(\frac{\rho_{\tau-1}^2}{30}\leq \frac{1}{2}\times\pi (\rho_{\tau-1}\times\frac{2-\sqrt{3}}{\sqrt{3}})^2\) and we get packing for all the small circles in \(\mathcal{C}_{S}^*\) along with the existing packing a subset of large circles \(\mathcal{C}_{L}^*\) in \(P^+\).

In this case we analyze the weight of final packing \(P^*\) in comparison of \(P\) in different cases: 

\[
w(P^*) = 
\begin{cases}
\lvert \mathcal{C}_{L}^* \rvert+\lvert \mathcal{C}_{S}^* \rvert, &  \lvert \mathcal{C}_{L}^* \rvert=1 \\
\lvert \mathcal{C}_{L}^* \rvert+\lvert \mathcal{C}_{S}^* \rvert, & \lvert \mathcal{C}_{L}^* \rvert=2 \text{ and } \lvert \mathcal{C}_{S}^* \rvert= 1
\\
3, &\lvert \mathcal{C}_{L}^* \rvert=2 \text{ and } \lvert \mathcal{C}_{S}^* \rvert= 2 \text{ or } 3 \\
\lvert \mathcal{C}_{L}^* \rvert-1 + \lvert \mathcal{C}_{S}^* \rvert,& \lvert \mathcal{C}_{L}^* \rvert=2 \text{ and } \lvert \mathcal{C}_{S}^* \rvert\geq 4 \\
3+\lvert \mathcal{C}_{S}^* \rvert, & 3 \leq \lvert \mathcal{C}_{L}^* \rvert \leq 5
\\
\lceil\frac{3}{4}\cdot\lvert \mathcal{C}_{L}^* \rvert\rceil-1+\lvert \mathcal{C}_{S}^* \rvert & 6 \leq \lvert \mathcal{C}_{L}^* \rvert

\end{cases}
\]

In this case our packing \(P^*\) has profit \(\geq \frac{3}{5}\OPT\) for all the subcases

\textbf{Case - II : } \(A_{\text{small}} > A_{\text{large}}\times \frac{\rho_{\tau-1}^2}{30}\)

When the number of small circles in \(P\) is much more compared to number of big circles in \(P\), we can get large profit by packing only the small circles even after discarding the large circles. We will use this idea in this scenario. Let's denote the number of small circles and large circles in \(P\) as \(n_{\text{small}}\) and \(n_{\text{large}}\). We have \(\sum_{c_{i} \in \mathcal{C}_{S}^*} a_{i} \geq (\sum_{c_{i} \in \mathcal{C}_{L}^*} a_{i})\times \frac{\rho_{\tau-1}^2}{30}\). We try to find the bound on minimum value of the ratio \(\frac{n_{\text{small}}}{n_{\text{large}}}\). Denote the circles in \(\mathcal{C}_{S}^*\) as \(\mathcal{C}_{S}^*=\{C_{s_{1}},C_{s_{2}},C_{s_{3}},...,C_{s_{n_{\text{small}}}}\}\) and circles in \(\mathcal{C}_{L}^*\) as \(\mathcal{C}_{L}^*=\{C_{l_{1}},C_{l_{2}},C_{l_{3}},...,C_{l_{n_{\text{large}}}}\}\) 

Note that \[A_{\text{small}}=\sum_{i=1}^{n_{\text{small}}} a_{s_{i}}\] 
and all the circles in \(\mathcal{C}_{S}^*\) have radius \(\leq \rho_{\tau}\). For a fixed \(A_{\text{small}}\) and among all the possible candidate sets of \(\mathcal{C}_{S}^*\), \(n_{\text{small}}\) will be minimum when all the circles in \(\mathcal{C}_{S}^*\) have radius \(\rho_{\tau}\). Hence we can bound \(n_{\text{small}}\) as \[n_{\text{small}} \geq \frac{A_{\text{small}}}{\pi \rho_{\tau}^2} \]
Also
\[A_{\text{large}}=\sum_{i=1}^{n_{\text{large}}} a_{s_{i}}\] 
and all the circles in \(\mathcal{C}_{L}^*\) have radius \(\geq \rho_{\tau-1}\). For a fixed \(A_{\text{large}}\) and among all the possible candidate sets of \(\mathcal{C}_{L}^*\), \(n_{\text{large}}\) will be maximum when all the circles in \(S^*\) have radius \(\rho_{\tau-1}\). Hence we can bound \(n_{\text{large}}\) as \[n_{\text{large}} \leq \frac{A_{\text{large}}}{\pi \rho_{\tau-1}^2} \]
Also note that

\begin{align*}
A_{\text{small}} &> A_{\text{large}}\times \frac{\rho_{\tau-1}^2}{4}\\
\Rightarrow n_{\text{small}}\times \pi \rho_{\tau}^2 &\geq n_{\text{large}} \times \pi \rho_{\tau-1}^2 \times \frac{\rho_{\tau-1}^2}{30} \\
\Rightarrow \frac{n_{\text{small}}}{n_{\text{large}}} &\geq \frac{\rho_{\tau-1}^4}{30\rho_{\tau}^2}
\end{align*}

Also we know that 
\begin{align*}
\rho_{\tau} &= \frac{1}{2} \times \rho_{\tau-1}^2\eps 
\Rightarrow \frac{\rho_{\tau-1}^4}{4\rho_{\tau}^2} = \frac{1}{\eps^2} \\
\Rightarrow \frac{n_{\text{small}}}{n_{\text{large}}} &\geq \frac{1}{8{\eps}^2} 
\Rightarrow n_{\text{large}} \leq 8\eps^2 \times n_{\text{small}}
\end{align*}
As the number of large circles in \(\mathcal{C}_{L}^*\) is much less compared to the number of small circles in \(\mathcal{C}_{S}^*\) and all the circles have unit profit, we choose to pack only the small circles. We remove all the large circles from \(\mathcal{C}_{L}^*\) that we have already packed in the bin. We continue only with the small circles in \(\mathcal{C}_{S}^*\) and pack these using $\mathtt{greedyNFDR}$ for unit profit circles in our optimal solution. Our final packing \(P^*\) will have weight \((\frac{\pi}{4}(1-4\rho_{\tau})-\pi\rho_{\tau}^2)\lvert \mathcal{C}_{S}^* \rvert\geq (\frac{\pi}{4}(1-4\rho_{\tau})-\pi\rho_{\tau}^2)\frac{(1-\eps)}{(1+8\eps^2)}w(\OPT)\geq(\frac{\pi}{4}(1-4\frac{\eps}{8})-\pi(\frac{\eps}{8})^2)\frac{(1-\eps)}{(1+8\eps^2)}w(\OPT)\geq\frac{3}{5}w(\OPT)\) as \(\eps \leq 0.1\).

\begin{theorem}
	\label{thm:5/3-apx}
	There is a polynomial time 5/3-approximation algorithm for the unweighted $\mathsf{CSK}$ problem in two dimensions.
\end{theorem}
\begin{proof}
	First we divide our set $\mathcal{C}$ of circles into intervals as described in section \ref{partiotion section}. After the intervals are produced, we will consider each as of the first \(\lceil\frac{1}{\eps}\rceil\) intervals as medium separately and produce a packing as per the structure as defined above. This approach will produce a finite number of packings and we can compare all of them and then return the one with the highest weight.
	We do the following for all \(\tau\) such that \(1 \leq \tau \leq \frac{1}{\eps}\).
	For \(\tau = 1\), we essentially have only medium and small circles. We discard the medium circles and pack a set of small circles using $\mathtt{greedyNFDR}$ as described in lemma \ref{greedyNFDR_lemma}. Essentially this case corresponds to when \(\mathcal_{C}_{L}^*=\emptyset\) and as described in section \ref{Big_Circle_Pack} this strategy gives us $\frac{5}{3}$-approximation.
	For \(\tau \neq 1\), we have all three type of circles and we call the of large circles as \(\mathcal{C}_{L}\), the set of medium circles as \(\mathcal{C}_{M}\) and the set of small circles as \(\mathcal{C}_{S}\). First we note that all the circles in \(\mathcal{C}_L\) have radius \(\geq \rho_{\tau-1}\) and area \(\geq \pi \rho_{\tau-1}^2\). Hence in an optimal packing there can be at most \(\frac{1}{\pi \rho_{\tau-1}^2}\) in any feasible packing. We guess the large circles in \(\OPT\) in \(n^{\left(\frac{1}{\pi\rho_{\tau-1}^2}\right)^{\mathcal{O}(1)}} \)time which is essentially \(n^{({\frac{1}{\eps}})^{\mathcal{O}(1)}}\) time since \(\rho_{\tau-1}\) is bounded by \(\eps\). We can guess the \(\mathcal{C}_{L}^*\) by exhausting all the possible feasible packing. If we find any circle in \(\mathcal{C}_{L}^*\) has diameter \(\geq 1-2\rho_{\tau-1}\), then we simply discard this circle from the set \(\mathcal{C}\) and pack other circles in $\mathcal{C}$ using $\mathtt{greedyNFDR}$ as described in lemma \ref{greedyNFDR_lemma} as described in section \ref{Big_Circle_Pack} this strategy gives a packing weight \(w(\OPT)-1\). If no such circle exist then we follow the steps as described in section \ref{Big_Circle_Pack} and modify the packing to get the structure \(P^+\). We further use the ideas of section \ref{Small-Circle-Pack} to pack the small circles from the set \(\mathcal{C}_{S}\) where we choose greedily the circles with smaller radius from the set \(\mathcal{C}_S\) and arrive at the final packing \(P^*\). Note that choosing greedily the smaller circles from \(\mathcal{C}_{L}\) we either guess all or more circles from \(\mathcal{C}_{L}^*\) which essentially means our packing weight is at least as much as of the final packing \(P^*\) as in section \ref{Small-Circle-Pack}. We separately deal with the case when the number of small circles is much greater than the number of large circles. In this case we only pack the circles in \(\mathcal{C}_{S}\) using greedyNFDR in the unit bin. 
	Finally our algorithm returns the packing with the maximum weight among all the packings generated in polynomial time and from our analysis it follows that the best packing has profit at least \(\frac{3}{5}\cdot w(\OPT)\).
\end{proof}
\end{comment}

==> append2.tex <==
% \section{Appendix}
% \label{sec:append}



\section{Improving the precision of the large spheres}
\label{subsec:Improve_Large} Recall that for each large circle $C_{i}\in\C_{L}^{*}$
we guessed its center in the optimal packing up to a polynomial error
of $\frac{\eps}{n}$. We improve this to only an exponential error
of at most $\frac{1}{2^{n/\eps}}$. To do this, we apply Theorem~\ref{thm:GrigorevVV88}
with $\alpha:=\Theta(\frac{1}{2^{n/\eps}})$. This yields more precise
estimates $\bar{x}_{i}^{(1)},\bar{x}_{i}^{(2)}$ for each $C_{i}\in\C_{L}^{*}$.
There is an important subtlety though: for our guessed coordinates
$\tilde{x}_{i}^{(1)},\tilde{x}_{i}^{(2)}$ we can assume that they
differ from the coordinates of $\OPT$ by at most our polynomial error
of $\frac{\eps}{n}$. For the new estimates $\bar{x}_{i}^{(1)},\bar{x}_{i}^{(2)}$
we can \emph{not }guarantee this: our subroutine from Theorem~\ref{thm:GrigorevVV88}
possibly returns a solution that is (close to) a feasible for the
large circles, but not (close to) a solution that is feasible for
the large and for the small circles. Because of this, we guessed the estimates
$\tilde{x}_{i}^{(1)},\tilde{x}_{i}^{(2)}$ for each $C_{i}\in\C_{L}^{*}$,
so that we can assume that these estimates really correspond to $\OPT$
and not just to some arbitrary solution to \eqref{eq:equations}.

If it were true that there is always a $(1+\eps)$-approximate solution
in which the center of each circle has rational coordinates that can
be encoded with a polynomially bounded number of bits, then we could
choose $\alpha$ appropriately to compute it. More precisely, we could
compute a range for each coordinate that contains only one rational
number with a bounded number of bits, and we could compute this number
afterward.



%
%
% \label{subsec:Improve_Large}
% So far, for each large circle $C_{i}\in\C_{L}^{*}$ we guessed values
% $\tilde{x}_{i}^{(1)},\tilde{x}_{i}^{(2)}\in\{0,\frac{\eps}{n},\frac{2\eps}{n},...,1\}$
% such that $\hat{x}_{i}^{(1)}\in[\tilde{x}_{i}^{(1)},\tilde{x}_{i}^{(1)}+\frac{\eps}{n})$
% and $\hat{x}_{i}^{(2)}\in[\tilde{x}_{i}^{(2)},\tilde{x}_{i}^{(2)}+\frac{\eps}{n})$.
% Hence, we possibly make a polynomial error of $\frac{\eps}{n}$.
% We improve this to only an exponential error of at most
% $\frac{1}{2^{n/\eps}}$. To do this, we apply Theorem~\ref{thm:GrigorevVV88} with
% $\alpha:=\Theta(\frac{1}{2^{n/\eps}})$. This yields more precise estimates
% $\bar{x}_{i}^{(1)},\bar{x}_{i}^{(2)}$ for each $C_{i}\in\C_{L}^{*}$.
% However, note that it
% might \emph{not} be the case that
% $\hat{x}_{i}^{(1)}\in[\bar{x}_{i}^{(1)},\bar{x}_{i}^{(1)}+\frac{1}{2^{n/\eps}})$
% and
% $\hat{x}_{i}^{(2)}\in[\bar{x}_{i}^{(2)},\bar{x}_{i}^{(2)}+\frac{1}{2^{n/\eps}})$
% for some $C_{i}\in\C_{L}^{*}$. The reason is that
% our system of inequalites~\eqref{eq:equations} can have solutions that differ from
% $\hat{x}_{i}^{(1)},\hat{x}_{i}^{(2)}$ for some (or even all) large circles $C_{i}\in\C_{L}^{*}$. Because of
% this, we guessed the estimates $\tilde{x}_{i}^{(1)},\tilde{x}_{i}^{(2)}$ for each $C_{i}\in\C_{L}^{*}$, so that
% we can assume that these estimates correspond to $\OPT$ and not just to some arbitrary solution to \eqref{eq:equations}.
%
% If it were true that there is always a $(1+\eps)$-approximate solution
% in which the center of each circle has rational coordinates that can be encoded with a polynomially bounded number of bits,
% then we could choose $\alpha$ appropriately to compute it. More precisely, we could compute a range for each coordinate that contains only one
% rational number with a bounded number of bits, and we could compute this number afterward.


\section{Shifting step}\label{sec:shifting}
%\begin{restatable}{lem}{shiftinglemmaapx}
\begin{lem}
	\label{lem:shifting}
	Let a given packing for a knapsack packing problem with input set \(\C\) of items be $\mathcal{P}$ and \(r\) be a total order on these objects and \(w_i\) be the weight associated with the \(i\)-th object. Let $\mathcal{C}_{\mathcal{P}}$ be the set of the items selected by $\mathcal{P}$ and we have $w(\mathcal{P}) = \sum_{C_{i}\in \mathcal{C}_{\mathcal{P}}} w_{i}$. Define $\rhoi{k} = h(\eps, k)$ where \(h\) is a given function. For each integer \(k\geqslant 1\), define the following sets of items:
	\(
	\mathcal{C}_k = \{C_i \in \mathcal{C} \mid r_{i} \in (\rho_{k},\rho_{k-1}]\}.
	\)
	Then there exists a \(\tau \leqslant \frac{1}{\eps}\) such that \(w(\C_{\tau}\cap\C_{\mathcal{P}})\leqslant\eps w(\mathcal{P})\).
\end{lem}
%\end{restatable}
\begin{proof}
We will partition the input set of $\mathcal{C}$ into large, medium, and small items using a partition function $\rho_k$ which we will design retrospectively after considering all the properties it needs to satisfy. The methodology is as follows, we partition the input $\mathcal{C}$ into several sets \(\mathcal{C}_k\)'s, and then select an appropriate index \(j \in [1/\eps]\) such that the sum of weights of all items from $\mathcal{P}$ in \( \mathcal{C}_j \leqslant \eps\cdot w(\mathcal{P})\) for a given constant $\eps>0$. We will declare this to be the medium items set $\mathcal{C}_M$ and discard it from $\mathcal{C}$.


Let $\eps>0$ be a positive real constant. We can assume that $\mathcal{P}$ has more than $\frac{1}{\eps}$ items. Otherwise, we can enumerate all the sets with at most \(\frac{1}{\eps}\) items. Among the selected items, we note \(r\) \ of the smallest item and let it be denoted as \(r_{\text{min}}\). For this selected set of items, we partition them with all the items categorized as large items and both the set of medium and small items as empty. Formally we define \(\mathcal{C}_L = \{C_{i} \in \mathcal{C} \mid r_{i}\geq r_{\text{min}}\}\) which contains all the items and then set \(\mathcal{C}_M\) and \(\mathcal{C}_S\) are empty.

Otherwise, we define $\rho_0=1$, and $\rhoi{k} := h(\eps, k) \cdot \rho_{k-1}$ where $h$ is the given function. For each integer $k \geqslant 1$ we define the following sets of items:
\begin{align*}
\mathcal{C}_k = \{C_i \in \mathcal{C} \mid r_{i} \in (\rho_{k},\rho_{k-1}]\}.
\end{align*}

Let $\tau$ be the smallest index such that the total weight, $w(\mathcal{C}_{\tau})$, of the items in $S_{\tau}$ is at most $\eps w(\mathcal{P})$. Observe that $\tau \leqslant \frac{1}{\eps}$ due to the pigeonhole principle. Partition the set $\mathcal{C}$ of items into three groups: the $\textit{large}$ items $\mathcal{C}_L = \{C_{i} \in \mathcal{C} \mid r_{i}>\rho_{\tau-1}\}$, the $\textit{medium}$ items $\mathcal{C}_M = \{C_{i} \in \mathcal{C} \mid \rho_{\tau} < r_{i} \leqslant \rho_{\tau-1}\}$ and the $\textit{small}$ items $\mathcal{C}_S = \{C_{i} \in \mathcal{C} \mid r_{i} \leqslant \rho_{\tau}\}$. Similarly, define sets $\mathcal{C}_L^* = \mathcal{C}_L \cap \mathcal{P}$, $\mathcal{C}_M^* = \mathcal{C}_M \cap \mathcal{P}$, and $\mathcal{C}_S^* = \mathcal{C}_S \cap \mathcal{P}$. Note that $\mathcal{C}_M^* = \mathcal{C}_{\tau}$, so the total weight of the medium items is at most $\eps\cdot w(\mathcal{P})$.
\end{proof}

\section{Omitted Proofs from Section~\ref{sec:ptas-ra}}
\begin{comment}
\subsection{Proof of \Cref{lem:fatdisc}}

	\begin{figure}%[H]
		\centering \includegraphics[width=1\textwidth]{Images/Final/aar_figure2.pdf}
		% 	\centering \includegraphics[width=0.3\textwidth]{Images/Final/corner}
		% Scale image to the width of the text
		\caption{\ag{Line $\Psi$ seperates the two $f$-fat and convex objects $P$ and $P'$. We construct line $\Upsilon$ such that it has intersects no common grid cells with line $\Psi$. We proceed to shrink the two objects $P, P'$ by a factor of $1+\eps$ such that they cannot intersect the space between lines $\Upsilon$ and $\Psi$.}}
		\label{fig:hyperplane}
	\end{figure}

	Let $P, P' \in \mathcal{P}$ be two $f$-fat convex $\dl$-large objects packed inside the knapsack.
	Then  by {\em separating hyperplane theorem for convex objects}~\cite{boyd2004convex}, we know that there is a line $\Psi$ containing a point $p_v$ on boundary of $P$, and $\Psi$ separates $P$ from $P'$  (see Figure \ref{fig:hyperplane}). 
	 Now, intuitively, increasing the size
	of the knapsack by a factor of $1+\eps$ is equivalent to shrinking
	the objects in $\mathcal{P}$ by a factor of $1+\eps$. So, we want find the right constraints such that after shrinking $P$ and $P'$ do not share any grid cell. 
	Let the center of the incircle (of radius $r^{in}$) contained in $P$ be $p_c$ and the line joining $p_c$ and $p_v$ be $\Lambda$. 
	Let the foot of the image of the point $p_c$ on line $\Psi$ be the point $p_z$.  Now the length of line segment $\overline{p_c p_z}  := |\overline{p_c p_z}| \geq r_{in}$ and $|\overline{p_c p_v}| \leq 2 f r_{in}$, due to fatness. Hence, the angle $\theta$ between $\Psi$ and $\Lambda$ is at least ${\sin}^{-1}(\frac{1}{2f})$. Consider points $p_x$ on $\Psi$ and $p_y$ on $\Lambda$ such that $|\overline{p_x p_y}| = \sqrt2 \dc$ and the line $\Upsilon$ joining $p_x, p_y$ is parallel to the line joining $p_c p_z$. %Let $\Upsilon$ be the line passing through $p_y$ and parallel to $\Psi$.  
	Then any point on $\Psi$ does not share a gridcell with any point on $\Upsilon$. 
	Also, $|\overline{p_y p_v}|  \le  2 \sqrt2 f \dc$.
	Now we want to shrink  $P$ by $(1+\eps)$ factor keeping $p_c$ at the same position such that the shrunk version of $P$ lies completely within one side of $\Upsilon$.
		After shrinking, $\overline{p_c p_v}$ gets smaller by $\eps |\overline{p_c p_v}| \ge \eps r^{in} \ge \eps \dl$.
		Now we choose $\dc$ such that $\dc \le \frac{\eps}{2 \sqrt2 f} \cdot \dl$.
	Thus we satisfy $\eps |\overline{p_c p_v}| \ge \eps \dl \ge  2 \sqrt2 f \dc  \ge  |\overline{p_y p_v}|$ and this ensures that the shrunk down version of $P$ and $P'$ do not share any grid cell.  
	We assign each polygon to the grid cells that it intersects with. 
	Hence this process leads to a discretization such that the no grid cell is intersected by two polygons.
	
	
\end{comment}	
	
	\begin{comment}
	Note that we have chosen the distance between $p_x,p_y$ such that they must lie in different grid cells. This means that the length of $y p_v$ can be at most $\sqrt2 f \cdot \dc$, which means that it can intersect with at most $\sqrt2 f$ grid cells.
	
	Consider a point $p_v$ on the boundary of $P$. Let the ray $\lambda$ join $p_c$, the center of in-circle (of $r^{in}$) contained in $P$, with $p_v$. We will first prove that $\lambda$ can intersect at most $\sqrt{2} f$ cells that intersect with the boundary of $P$ and are not completely contained in $P$.
	
	\ag{Using the seperating hyperplane theorem for convex objects (~\cite{sephyperplane}), we know that there is a line $h$ containing $p_v$ such that all objects other than $P$ intersecting the ray $\lambda$ are separated by $P$ by $h$.}
	\ag{Let the foot of the image of point $p_c$ on line $h$ be point $p_z$. Notice that distance$(p_c p_z) \geq r_{in}$ and distance$(p_c p_v) \leq f r_{in}$ due to fatness. Hence we get that the angle $\theta$ between $h$ and $\lambda$ is at least $\tan^{-1}(1/f)$.}
	\ag{Consider points $p_x$ on $h$ and $p_y$ on $\lambda$ such that $\ell(p_x p_y) = \sqrt2 \dc$ and $p_x p_y$ is parallel to $p_c p_z$. Note that we have chosen the distance between $p_x,p_y$ such that they must lie in different grid cells. This means that the length of $y p_v$ can be at most $\sqrt2 f \cdot \dc$, which means that it can intersect with at most $\sqrt2 f$ grid cells. Notice that all cells that intersect both $\lambda$ and the boundary of object $P$ must also intersect $p_y p_v$, so we get that there can be at most  $\sqrt2 f$ such grid cells for appropriate choice of $\dc,\dl$.}
	
	\ag{After shrinking by a factor of $\eps$ (effectively magnifying the knapsack by the same factor), $p_c p_v$ gets smaller by $\eps |p_c p_v| \ge \eps r^{in} \ge \eps \dl$.
	By choosing $\eps \dl \ge \sqrt2 f \cdot \sqrt{2} \eps \dc = 2f \eps \dc$ we can ensure that after shrinking $P$ the point $p_v$ is completely contained within cells which had no intersection with any other objects in $\mathcal{P}$. }\ag{Hence this magnifying(or object shrinking) process leads to a discretization such that the no grid cell is intersected by two polygons.
	}
	\end{comment}

\begin{comment}
By the classical Barbier's theorem, we know  the perimeter of a convex set $P$ is at most $\pi \cdot \text{diameter}(P) \le 2\pi r^{out} \le 2\pi f \cdot r^{in}$. Now we can break the perimeter into  $\lceil (2\pi f \cdot r^{in)}/ (\dc)  \rceil$ curved segments of length at most $\dc$. Each such segment can at most intersect with 9 grid cells. Hence, \aw{the} total area of the grid cells \aw{overlapping with} the perimeter of $P$ is at most $9 \lceil (2\pi f \cdot r^{in)}/ (\dc)  \rceil \times (\dc )^2 \leq 20\pi f \cdot r^{in} \dc$.
	Therefore,   $(\area(\mathcal{G}_P)-\area(P))/\area(P) \le  \frac{20\pi f r^{in} \dc }{\pi(r^{in}-2\dc )^2} \le  \frac{20\pi f \dl  \dc }{\pi(\dl  - 2\dc )^2}
	\le  \frac{20 f \dl \dc}{(\dl-2 \dc)^2}  \le \eps^2 \cdot \dl^2$, by choosing  $\dc \le \eps^2 \dl^3/ 320 f$.  \arir{check the calc}
	
	Hence, $\sum_P \area(\mathcal{G}_P)-\area(P) \le \sum_P \eps \area(P) \le \eps^2$.
	Thus, total area of gray cells where two convex sets can overlap is only $\eps^2$. For each overlapped cell, we translate by its length and total translation needed is at most $\eps$.	
	
	Assuming $\eps<1/160f$, we see that $\dc=\eps^6$ and $\dl=\eps$ work. Note that any two "overlapping" grid cells that both intersect a different set of polygons are at a distance of at least $\delta_{large}/2$ because all the polygons have an inradius of at least $\delta_{large}$. 
	Now $(\area(\mathcal{G}_P)-\area(P))/\area(P) \le \eps\cdot \dl^2/4$ guarantees that the total shift in the $x$-direction will be at most $\eps$ because there can be at most $4/\dl^2$ many overlapping cells, causing a shift of at most $4\dc/\dl^2$.
\end{comment}

\subsection{Proof of \Cref{lem:medium-items}}
\arir{check this. The proof was missing earlier. Aaryan, can you find exact $\beta$ and $\gamma$ from other required conditions.
For example, $\gamma \le \eps/ 2 \sqrt{2} f$ from Lemma 2.}
This follows from a shifting argument similar to Lemma \ref{lem:shifting}. 
Say, we need $\ds \le \dc \le \dl$ such that $\ds \le \beta \dc, \dc \le \gamma \dl$, for some constants $\beta, \gamma \in (0,1]$. 
Define $\rho_0 := 1$, %(\beta \gamma)^{1/\eps} \cdot \eps/f$, 
and $\rhoi{k} := \beta \gamma \cdot \rho_{k-1}$. For each integer $k \in [2/\eps]$ 
\arir{to make sure $\dl, \dc$ is sufficiently small such that medium items have small radius and can fit in the augmented region of $\eps$ width. Another simpler option might be just to show area of medium to be $\eps^2$ instead of $\eps$, by using more classes.
We can also start with $\rho_0=\eps^2$ but then $\delta_{c,\ell} \neq \dc \delta_{c,\ell-1}$ for all $\ell$.}
we define the following sets of items as shown in \Cref{fig:split}:
\begin{align*}
\mathcal{C}_k = \{C_i \in \mathcal{P} \mid r^{in}(C_i) \in \bigcup_{j=1}^{\infty} (\rho_{k},\rho_{k-1}]\cdot (\beta \gamma)^{(2j/\eps)}\}.
\end{align*}
\begin{figure}%[H]
	\centering \includegraphics[width=\textwidth]{Images/Final/aar_figure4}
	% Scale image to the width of the text
	\caption{Splitting of sets $\mathcal{C}_k$ on the real line as used in \Cref{lem:medium-items}.}
	\label{fig:split}
\end{figure}
Then, by averaging argument there is a $k \in \{\frac{1}{\eps}+1, \frac{1}{\eps}+2, \cdots, \frac{2}{\eps}\}$  such that the area of $\mathcal{C}_k$ is at most $\eps$.
Define $\dl:=\rho_{k-1}, \dc:=\gamma \dl, \ds:=\beta \dc=\beta \gamma \dl=\beta \gamma \rho_{k-1}=\rho_k$. 
Define $D:= \{{(\beta \gamma)}^{2/\eps}, {(\beta \gamma)}^{2/\eps -1 }\gamma, {(\beta \gamma)}^{(2/\eps)-1}, \dots,  (\beta \gamma)^{1/\eps+1},  (\beta \gamma)^{1/\eps} \gamma, (\beta \gamma)^{1/\eps})\}$.
Clearly, any chosen $\ds, \dc, \dl$ belong to $D$.
Also, as $k \in \{\frac{1}{\eps}+1, \frac{1}{\eps}+2, \cdots, \frac{2}{\eps}\}$, we have $\dc,\dl \le {(\beta \gamma)}^{1/\eps}$. 

Later we will see that choosing \ag{$\beta=\eps^2/16, \gamma=\eps/(72f)$} suffices for our purpose (see proof of \Cref{lem:fatdiscrete}). 
This also ensure that any object in $\cup_{\ell} M_\ell$ has outradius (and thus inradius)  at most $\eps$. 

%Also, this ensures their area is at most $\eps$.
 
%Let us define \ag{ $\rho_{k,l} = \eps^{10} \cdot  \rho_{k-1,l}$ }with $\rho_{0,l}= \delta_{small,l}$. 
% For level $l$, define the set $b_{k,l}$ to be the set of all polygons with $\rho_{k,l} \leq r_{in} < \rho_{k-1,l}$. Now define the buckets \ag{$B_{k}= \bigcup_{l=1}^{l=\infty} b_{k,l}$}. We apply our standard shifting argument from \Cref{lem:shifting} and we are guaranteed to find a set of items $B_k$ that has an area of at most $\eps$ with $k= O_{\eps}(1)$. This is our set of medium circles corresponding to the chosen parameters. 
\begin{comment}
\subsection{Proof of \Cref{lem:fatdiscrete}}
We start with the given packing of $\mathcal{P}$ in $K$ and do a
sequence of refinements which leads to our discretized packing for
$\mathcal{P}\cap\bigcup_{\ell}L_{\ell}$. First, we use the increased
size of the knapsack to ensure that for each level $\ell$ and any
two objects $P,P'\in L_{\ell}$, the distance between $P$ and $P'$
is at least $2\delta_{c,\ell}$. Intuitively, increasing the size
of the knapsack by a factor of $1+\eps$ is equivalent to shrinking
the objects in $\mathcal{P}$ by a factor of $1+\eps$. Therefore,
we can achieve this required minimum distance of $2\delta_{c,\ell}$
by choosing $\dc$ \ag{appropriately acoording to the multiple constraints given in the proof of  \Cref{lem:fatdisc}}.

%Consider a point $p_v$ on the boundary of $P$. A line $l$ joining $p_v$ with $p_c$, the center of in-circle (of $r^{in}$) contained in $P$, can intersect at most $O_f(1)$ cells that intersect with the boundary of $P$ and are not completely contained in $P$.
%This follows from the $f$-fatness and convexity property of $P$. 
%After shrinking $l$ gets smaller by $\eps |l| \ge \eps r^{in} \ge \eps \delta_{large,\ell}$.
%By choosing $\eps \delta_{large,\ell} \ge O_f(1) \cdot \sqrt{2} \eps \delta_{cell,\ell}$ we can ensure that after shrinking $P$ the point $p_v$ is completely contained within cells which had no intersection with any other objects in $\mathcal{P}$.


Next, we would like that for each level $\ell$, each object in $\mathcal{P}\cap L_{\ell}$
is contained in a grid cell of level $\ell-1$. This might not be
the case, however, via a shifting argument (giving the grid a random
shift) we can argue that this is the case for almost all objects in
$\mathcal{P}$.
\ag{The probability that an object in level $\ell$ intersects a grid line from level $\ell-1$ is at most \ari{$8\delta_{small,\ell-1}/\delta_{cell,\ell-1}= 8\ds/\dc$}.
Let this probability be smaller than $\eps^2/2$, leading to a constraint \ari{$\ds \leq \eps^2\dc/16$} on the choice of $\dc,\ds$. Then the total area of intersecting objects must also be smaller than $\eps^2$ as the area of all packed objects can be at most the area of augmented knapsack.
}
%Due to our shifting argument, all other objects in
%$\mathcal{P}$ have a total area that is very small \ag{(at least $\eps$ fraction)} compared to the
%size of the knapsack and, thus, 
Thus we can easily pack these intersected objetcs into extra
space that we gain via increasing the size of the knapsack (i.e.,
for a second time).

After this preparation, we process the objects $P\in\mathcal{P}$
level by level and define their corresponding sets $\mathcal{G}_{P}$,
starting with the highest level. Consider a level $\ell$. For each
object $P\in\mathcal{P}$ of level $\ell$ we define $\mathcal{G}_{P}$
to be the set of all grid cells of level $\ell$ that intersect with
$P$. Due to our minimum distance between any two objects in $\mathcal{P}$
of level $\ell$, for any two different objects $P,P'\in\mathcal{P}$
of level $\ell$ we have that $\mathcal{G}_{P}\cap\mathcal{G}_{P'}=\emptyset$.
Now it could be that a cell $C\in\mathcal{G}_{P}$ for some $P\in\mathcal{P}$
intersects not only with $P$, but also with another object $P'\in\mathcal{P}$
of some deeper level $\ell'>\ell$. We call such a cell $C$ \emph{problematic};
recall that we wanted the cells in $\mathcal{G}_{P}$ to be used exclusively
by $P$. Therefore, we move all objects $P'\in\mathcal{P}$ of some
level $\ell'>\ell$ that intersect a problematic grid cells in $\mathcal{G}_{P}$.
We pack them into extra space that we gain due to resource augmentation.
We do this operation for all levels $\ell$.

In the process above, we move objects that intersect problematic grid
cells. We need to argue that the total area of these moved objects
is small compared to the size of the knapsack and that, therefore,
we can pack them into additional space that we gain due to our resource
augmentation. In particular, we need to argue this globally, over
all levels. The key insight is that if we define a set $\mathcal{G}_{P}$
for some object $P\in\mathcal{P}$ as above, then each problematic
cell $C\in\mathcal{G}_{P}$ must intersect the boundary of $P$ and,
since $P$ is fat, the number of problematic cells $C\in\mathcal{G}_{P}$
is very small compared to the number of cells $C'\in\mathcal{G}_{P}$
that are contained in $P$ and, thus, for sure \emph{not }problematic.

\arir{Check these calculations}
\ari{By the classical Barbier's theorem, we know  the perimeter of a convex set $P$ of level $\ell$ is at most $\pi \cdot \text{diameter}(P) \le 2\pi r^{out} \le 2\pi f r^{in}$.}
\ag{A curve of length $\dc$ is bound to be contained inside a circle of radius $\dc$. This implies that this curve can intersect at most $9$ grid cells as any circle of radius $\dc$ can be bound in a $3\times 3$ grid square.}
\ag{
Hence, the number of grid cells (of level $\ell$) $N_1$ that the perimeter can intersect is at most $18\pi f r^{in}/\delta_{cell,\ell}$. }
\ari{
On the other hand, $P$ completely contains at least grid cells of area $\pi (r^{in}-2\delta_{cell, \ell})^2$, 
i.e., the number of such gridcells $N_2$ is at least $\frac{\pi (r^{in}-2\delta_{cell, \ell})^2}{(\delta_{cell, \ell})^2}$.
We need $N_1 \le \eps N_2$.}
\ag{Equivalently, we want to show, $\delta_{cell, \ell} \le \frac{\eps}{18f} \cdot \frac{(r^{in}-2\delta_{cell, \ell})^2}{r^{in}}$.
For this we impose the condition that $\dl \ge \frac{72f}{\eps} \dc$.
Then, $\frac{\eps}{18f} \cdot \frac{(r^{in}-2\delta_{cell, \ell})^2}{r^{in}} \ge \frac{\eps}{18f} \cdot \frac{(r^{in}/2)^2}{r^{in}}\ge  \frac{\eps}{18f} \cdot \frac{\delta_{large, \ell}}{4} \ge \delta_{cell, \ell}$.}

%\ge \pi (\delta_{large,\ell}-2\delta_{cell, \ell})^2$, i.e., the number of such gridcells is at least 
%$(\pi (\delta_{large,\ell}-2\pi \delta_{cell, \ell})/\delta_{cell,l})^2 \ge \pi(\frac{\dl}{\dc}-2)^2 \ge \pi(\frac{\dl}{2\dc})^2$ by assuming $\dl \ge 4\dc$.
%Hence, we require $(2 f /\dc) \le \eps (\frac{\dl}{2\dc})^2$
%to ensure that the area of  problematic cells for an object $P$ is $\eps$ factor smaller than the cells completely contained in $P$
%We obtain this by the setting .}


Using this, we derive a \emph{global }argumentation, stating that
the total area of \emph{all} problematic grid cells over all objects
of all levels is at most an $\eps$-fraction of the area of the
knapsack. Also, if an object $P'$ of some level $\ell'$ intersects
a problematic grid cell $C$ of some level $\ell<\ell'$, then $P'$
is very small compared to $C$. Thus, the total area of these objects
intersecting a problematic grid cell $C$ is essentially the same
as the area of $C$. Thus, we can pack all these objects into our
additional space due to resource augmentation.

Finally, we can afford to increase the space of our knapsack such
that this additional space is even by a constant factor larger than
the total area of the objects we need to pack into it. Therefore,
it is easy to find a discretized packing for them in this extra space.
\end{comment}
\subsection{Proof of \Cref{lem:med}}
\arir{Check this proof}
Let the most profitable subset of $\bigcup_{\ell} \tilde{M}_{\ell}$
(up to a factor of $1+\eps$) whose total area is bounded by $\eps$ be $OPT_{M}$.
 We arrange all items in $\bigcup_{\ell}\tilde{M}_{\ell}$ in order of decreasing profit density and select (prefix) subset of items with higest profit density such that their area is bounded by $2\eps$. Let this subset of items be $M'$. We argue that $w(M')\ge w(OPT_M)$ as any items in $\bigcup_{\ell} \tilde{M}_{\ell}$ has area at most $\eps$.
 Therefore, our selected set $M'$ is has profit at least $\profit(\bigcup_{\ell}M_{\ell})$
(see Lemma~\ref{lem:medium-items}).
Now we pack  $M'$ 
separately in a strip of the form $[0,1]\times[1,1+O(\eps)]$.
% ,
% i.e., the area of the strip $[0,1]\times[1,1+\eps]$.
We replace each
of these objects by the smallest square that contains it, which
increases its area only by a constant factor of at most {$2f^2$ since each item is $f$-fat. Note that this square has a side length of at most $2r^{out} \le 2f r^{in} \le 2f\eps$ as all the medium objects have an inradius of at most $\eps$. Now we state a result that gives an approximation algorithm for packing small squares of size $O(\eps$) efficiently.}
\begin{lemma}[\cite{NFDH}]\label{lem:nfdh}
	In a rectangle of size $a \times b$, the $\mathtt{NFDH}$ algorithm guarantees to pack an area of at least $(ab-\mu(a+b))$ with sufficient number of squares of maximum side length $\mu$.
\end{lemma}

We pack these square objects greedily with the $\mathtt{NFDH}$ algorithm
\cite{NFDH} stated in \Cref{lem:nfdh} into a (slightly larger) strip $[0,1]\times[1,1+O_f(\eps)]$ to arrive at the result we wanted to prove.

\subsection{Proof of \Cref{lem:small-poly}}
We begin by assuming that the optimal solution for this problem is $\OPT$. We then remove two randomized strips of width $\eps$, and incur an (expected) loss of at most $2(2 r^{out}+\eps) \le 6 \eps$ fraction of the profit. 
This can also be derandomized by an averaging argument. 
From this, we get a packing of $(1-O(\eps)) \ag{w(\OPT)}$ profit in a $(1-\eps)\times (1-\eps)$ bin. We now use Theorem~\ref{thm:fat-ra} to get this packing from the set $\P$ in polynomial time. 

\section{Omitted Proofs from \Cref{sec:spheres}}

\subsection{Proof of \Cref{lem:create-gap}}
\begin{proof}
We set $f(x)=x^{24}$ in \Cref{lem:shifting} and immediately get the required result.
\end{proof}
\subsection{Proof of \Cref{big_sol}}
\begin{proof}
	Each large circle has area $\pi \epsl^2$. Thus there can be at most $1/(\pi \epsl^2)= 1/(\pi ({\eps^{{24}^k})^2})$ large circles. 
\end{proof}
\subsection{Proof of \Cref{lem:small-circles-grid-cells}}
	
\begin{proof}
	For each horizontal (resp. vertical) gridline $\ell$, each $C \in \mathcal{C}_{cut}$ must lie in a strip of height (resp. width) $4\epss$ and width (resp. height) 1. Totally there are $2/\epsc$ gridlines.
	Thus $\area(\mathcal{C}_{cut}) \leqslant 8 \epss/\epsc = 8 \epsl^{12}  \leqslant  \eps \epsl^2/64$. The last inequality follows from the fact that $\epsl \leqslant \eps \leqslant 1/2$.
\end{proof}

\subsection{Proof of \Cref{lem:gray-circles}}

\begin{figure}[ht]
	\begin{center}
		\includegraphics[width=5cm]{Images/Final/email-figure-4-final.pdf}
		\caption{Three types of cells for a particular circle}
		\label{fig:gray_cell_partition_types}
	\end{center}
\end{figure}
\begin{proof}
	Consider a large circle $C_L$ with radius $r_L \geqslant \epsl$. Let $\G_{g, C_L}, \G_{b, C_L}$ the set of gray and black grid cells that overlap with $C_L$.
	We will first show that $\G_{g, C_L}$ is much smaller compared to  $\G_{b, C_L}$.
	Note that for $C_L$,  we only have an estimate $\tilde{x}_{C}^{(1)},\tilde{x}_{C}^{2}$ of the coordinate of its center up to
	a \emph{polynomially} small error of $\eps/n$. 
	
	First we claim that all the cells intersected by a circle centered at  $(\tilde{x}_{C}^{(1)},\tilde{x}_{C}^{2})$ of radius $r_L- 3\epsc$ are in $\G_{b, C_L}$. 
	For contradiction, assume there is a gray cell $S_g$ intersected by a circle $C$ centered at  $(\tilde{x}_{C}^{(1)},\tilde{x}_{C}^{2})$ of radius $r_L- 3\epsc$.
	Then, the distance of any point in $S_g$ from the center of the circle is at most $r_L- 3\epsc +\sqrt{2\epsc} < r_L-\eps/n$. Thus  $S_g$  is completely contained within $C$.
	
	Similarly, we can show that the cells that are outside of a circle centered at  $(\tilde{x}_{C}^{(1)},\tilde{x}_{C}^{2})$ of radius $r_L+ 3\epsc$ are not in $\G_{b, C_L}$.
	
	Hence, $\area(\G_{b, C_L}) \geqslant \pi (r_L- 3\epsc)^2$ and $\area(\G_{g, C_L}) \leqslant \pi (r_L+3\epsc)^2 - \pi(r_L-3\epsc)^2=12 \pi \epsc r_L$.
	Hence, 
	\[
	\frac{\area(\G_{g, C_L})}{\area(\G_{b, C_L})} \leqslant \frac{12 \pi \epsc r_L}{\pi (r_L- 3\epsc)^2} \leqslant \frac{12 \epsc r_L}{(r_L/2)^2} \leqslant 48\frac{\epsc}{\epsl} = 48 \epsl^{11} \leqslant \eps \epsl^2/5
	\]
	The second inequality follows from the fact that $\epsl \leqslant \eps \leqslant 1/2$ and $r_L \geqslant \epsl$.  The last inequality uses the fact that $\eps \leqslant 1/2$.
	Therefore, $\sum_{C \in \C_{L}^{*}} {\area(\G_{g, C_L})} \leqslant (\eps \epsl^2/5) \cdot \sum_{C \in \C_{L}^{*}}  {\area(\G_{b, C_L})} \leqslant \eps \epsl^2/5$.
\end{proof}

\subsection{Proof of \Cref{lem:white-circles}}
\begin{figure}[ht]
	\begin{center}
		\includegraphics[width=6cm]{Images/Final/email-figure-2-3.pdf}
		\caption{(a)The square \(S_w\) and the large circle \(C\) (b) Orientation of circle \(C\) after translation}
		\label{fig:corner_cell}
	\end{center}
\end{figure}

\begin{proof}
	In \Cref{fig:corner_cell}, consider a corner (w.l.o.g., left bottom corner) $v_{lb}$ of the knapsack. Let  $S_w$ be a square region of side length $\epsl/4$ such that $S_w$ is contained in the knapsack and shares $v_{lb}$.
	We will show that no large circles intersect $S_w$ and thus all grid cells in $S_w$ are white.
	
	For contradiction, assume that some large circle $C$ intersects $S_w$. As $r_C \geqslant \epsl$, if $C$ intersects either the top or right edge of $S_w$ it must intersect the top right corner of $S_w$ at $(\epsl/4, \epsl/4)$.  Thus, $(\epsl/4, \epsl/4)=: v_{trw} \in C$. 
	Then consider $C$ in the knapsack and we can move $C$ towards $v_{lb}$  such that it touches two boundary edges of the knapsack, i.e.,  the center of $C$ is now at $(r_C, r_C)$. Note that, after this translation, $C$ should continue to intersect $S_w$, i.e.,  $(\epsl/4, \epsl/4) \in C$. 
	However, distance of $v_{trw}$ from $(r_C, r_C)$ is $\sqrt{(r_C-\frac{\epsl}{4})^2 + (r_C-\frac{\epsl}{4})^2} \geqslant \sqrt{2(\epsl-\frac{\epsl}{4})^2} > \epsl$.
	Thus,  $v_{trw} \notin C$. This is a contradiction. 
	
	Now, we can argue this analogously for all the corners of the knapsack and the lemma is proved. 
\end{proof}



\subsection{Proof of \Cref{thm:d-dim-ptas}: \textsf{PTAS} for $d$-dimensional hyperspheres}

	In order to extend out techniques to \(d\)-dimension, we start with first creating partitions over the \(d\)-dimensional hyperspheres by setting \(f(x)=x^{12d}\) in \Cref{lem:shifting} and \(\eps^{j}=(\eps^{j-1})^{12d}\) in  \Cref{lem:create-gap}
	
	Further, we notice that each large hypersphere has volume at least \( \dfrac{\pi^{\frac{d}{2}}}{\Gamma\left(\frac{d}{2} + 1\right)} \cdot \epsl^d
	\). Thus, there can be at most \(\dfrac{1}{\frac{\pi^{\frac{d}{2}}}{\Gamma\left(\frac{d}{2} + 1\right)} \cdot \epsl^d}\) large hyperspheres in any feasible solution. Using the techniques as in \Cref{subsec:Large_Guess}, we can guess and verify the coordinates of the large hyperspheres in \(\mathcal{C}_{L}^*\) in polynomial time. Also observe that the guessed values $\tilde{x}_{i}^{(1)},\tilde{x}_{i}^{(2)},\dots,\tilde{x}_{i}^{(d)}$
	yield an estimate for $\hat{x}_{i}^{(1)},\hat{x}_{i}^{(2)},\dots,\hat{x}_{i}^{(d)}$ up to a (polynomially small) error of $\eps/n$
	
	In order to find a feasible packing of the small hyperspheres we will replicate techniques from \Cref{subsec:placing_small}.  Define \(\epsc:=\epsl^{6d}\)(i.e, \(\epss=\epsl^{12d}=\epsc^2\)). To subdivide the knapsack into \(1/\epsc^d\) $d$-dimensional grid cells of length \(\epsc\). We denote a grid cell by \(G_{\ell^{(1)},\dots,\ell^{(d)}}:=[\ell^{(1)}\cdot\epsc,(\ell^{(1)}+1)\cdot\epsc)\times\dots\times[\ell^{(d)}\cdot\epsc,(\ell^{(d)}+1)\cdot\epsc)\). We define the set of grid cells by \(\G:=\{G_{\ell^{(1)},\dots,\ell^{(d)}}:\ell^{(1)},\dots,\ell^{(d)}\in\{0,1,\dots,1/\epsc-1\}\}\) To proceed further, we first prove structural properties for the packing of the hyperspheres in the grids. For any set \(\mathcal{S}\) of circles or grid cells, we define \(\area(\mathcal{S})\) to be the total volume of the elements in \(\mathcal{S}\).
	\begin{lem}\label{lem:small-hypersphere-grid-cells}
		Let \(\mathcal{C}_{cut}\subseteq\C_{S}^{*}\) be the set of all small hyperspheres in \(\C_{S}^{*}\) that intersect more than one grid cell. We have that \(\area(\mathcal{C}_{cut})\leqslant4d\epss/\epsc\leqslant d\eps\epsl^d/2^{5d-3}\)
	\end{lem}
	\begin{proof}
		For each of the \(i\)-th dimension for \(1\leqslant i \leqslant d\), and for each of the gridline \(\ell\) in this dimension, each \(C\in\C_{cut}\) must lie in a strip with the \(i\)-th dimension being \(4\epss\) and all other dimensions being 1. Totally, there are \(d/\epsc\) gridlines. Thus, \(\area(\C_{cut})\leqslant4d\epss/\epsc=4d\epsl^{6d}\leqslant d\eps\epsl^d/2^{5d-3}\). The last inequality follows from the fact \(\epsl\leqslant \eps\leqslant 1/2\).
	\end{proof}
	We partition \(\G\) into \(\emph{white},\emph{black},\emph{gray}\) cells with respect to the position of the large hyperspheres similarly as the case of circles. We give bounds similar to \Cref{lem:gray-circles} and \Cref{lem:white-circles} in the case of $d$-dimensions for \emph{gray} and \emph{white} cells.
	\begin{lem}\label{lem:gray-circles-d}
		The total volume of gray cells \(\area(\G_{g})\) is at most \(\dfrac{(d+1)(3^d-1)\eps\epsl^d}{2^{5d-3}}\). We can compute \(\G_g\) in polynomial time.
	\end{lem}
	\begin{proof}
		Consider a large hypersphere \(C_L\) with radius \(r_L\geqslant\epsl\). Let \(\G_{g, C_L},\G_{b, C_L}\) be the set of gray and black grid cells that overlap with \(C_L\). Note that, for \(C_L\) we only have an estimate \(\tilde{x}_{C}^{(1)},\dots,\tilde{x}_{C}^{(d)}\) of the coordinate of its center up to a \(\emph{polynomially}\) small error of \(\eps/n\).
		
		First we claim that all the cells intersected by a hypersphere centered at  \((\tilde{x}_{C}^{(1)},\dots,\tilde{x}_{C}^{(d)})\) of radius $r_L- (d+1)\epsc$ are in $\G_{b, C_L}$. 
		For contradiction, assume there is a gray cell $S_g$ intersected by a circle $C$ centered at  \((\tilde{x}_{C}^{(1)},\dots,\tilde{x}_{C}^{(d)})\) of radius $r_L- (d+1)\epsc$.
		Then, the distance of any point in $S_g$ from the center of the circle is at most $r_L- (d+1)\epsc +\sqrt{d\epsc} < r_L-\eps/n$. Thus, $S_g$  is completely contained within $C$.
		
		Similarly, we can show that the cells that are outside of a circle centered at  \((\tilde{x}_{C}^{(1)},\dots,\tilde{x}_{C}^{(d)})\) of radius $r_L+ (d+1)\epsc$ are not in $\G_{b, C_L}$.
		
		Hence, 
		\begin{align*}
		\area(\G_{b, C_L}) &\geqslant \frac{\pi^{\frac{d}{2}}}{\Gamma\left(\frac{d}{2} + 1\right)} \cdot (r_L-(d+1)\epsc)^d \\
		\area(\G_{g, C_L}) &\leqslant \frac{\pi^{\frac{d}{2}}}{\Gamma\left(\frac{d}{2} + 1\right)} \cdot (r_L+(d+1)\epsc)^d - \frac{\pi^{\frac{d}{2}}}{\Gamma\left(\frac{d}{2} + 1\right)} \cdot (r_L-(d+1)\epsc)^d \\ 
		&\leqslant \frac{\pi^{\frac{d}{2}}}{\Gamma\left(\frac{d}{2} + 1\right)} \cdot 2(d+1)((3/2)^d-(1/2)^d)\epsc r_{L}^{d-1}
		\end{align*}
		\begin{comment}
		
		$\area(\G_{b, C_L}) \geqslant \dfrac{\pi^{\frac{d}{2}}}{\Gamma\left(\frac{d}{2} + 1\right)} \cdot (r_L-(d+1)\epsc)^d$, and\\ $\area(\G_{g, C_L}) \leqslant \dfrac{\pi^{\frac{d}{2}}}{\Gamma\left(\frac{d}{2} + 1\right)} \cdot (r_L+(d+1)\epsc)^d - \dfrac{\pi^{\frac{d}{2}}}{\Gamma\left(\frac{d}{2} + 1\right)} \cdot (r_L-(d+1)\epsc)^d\leq \dfrac{\pi^{\frac{d}{2}}}{\Gamma\left(\frac{d}{2} + 1\right)} \cdot 2(d+1)((3/2)^d-(1/2)^d)\epsc r_{L}^{d-1}$. 
		\end{comment}
		The inequality follows from the fact, \(r_{L}/2\geqslant(d+1)\epsc\)\\
		
		Hence we can bound the ratio of \(\frac{\area(\G_{g, C_L})}{\area(\G_{b, C_L})}\) as
		\[
		\begin{aligned}
		\frac{\area(\G_{g, C_L})}{\area(\G_{b, C_L})} &\leqslant \frac{\frac{\pi^{\frac{d}{2}}}{\Gamma\left(\frac{d}{2} + 1\right)} \cdot 2(d+1)((3/2)^d-(1/2)^d)\epsc r_{L}^{d-1}}{\frac{\pi^{\frac{d}{2}}}{\Gamma\left(\frac{d}{2} + 1\right)} \cdot (r_L-(d+1)\epsc)^d} \\
		&\leqslant \frac{2(d+1)((3/2)^d-(1/2)^d)\epsc r_{L}^{d-1}}{(r_L/2)^2} \\
		&\leqslant \frac{2(d+1)(3^d-1)\epsc}{r_L} \leqslant \frac{2(d+1)(3^d-1)\epsc}{\epsl} \\
		&= 2(d+1)(3^d-1)\epsl^{6d-1} \leqslant \frac{(d+1)(3^d-1)\eps\epsl^d}{2^{5d-3}}
		\end{aligned}
		\]
		
		Inequalities follow from the fact that $\epsl \leqslant \eps \leqslant 1/2$ and $r_L \geqslant \epsl$.  The last inequality uses the fact that $\eps \leqslant 1/2$.
		Therefore, $\sum_{C \in \C_{L}^{*}} {\area(\G_{g, C_L})} \leqslant \bigg(\dfrac{(d+1)(3^d-1)\eps\epsl^d}{2^{5d-3}}\bigg) \cdot \sum_{C \in \C_{L}^{*}}  {\area(\G_{b, C_L})} \leqslant \dfrac{(d+1)(3^d-1)\eps\epsl^d}{2^{5d-3}}$.
	\end{proof}
	\begin{lem}\label{lem:white-circles-d}
		The total volume of the white grid cells \(\area(\G_w)\) is at least \(\frac{\epsl^d}{2^d}\), We can compute \(\G_w\) in polynomial time.
	\end{lem}
	\begin{proof}
		Similarly arguing as in \Cref{lem:white-circles}, we can show that no hypersphere can intersect a $d$-dimensional bin of side length \(\epsl/4\) at each corner. Hence the total volume of white grid cells must be at least \(2^d\cdot(\epsl/4)^d=(\epsl/2)^d\)
	\end{proof}
	
	We note here that the total volume of gray cell and \(\C_{cut}\) is at most \(d\eps\epsl^d/2^{5d-3}+\dfrac{(d+1)(3^d-1)\eps\epsl^d}{2^{5d-3}} \leqslant \eps (\epsl/2)^d\). Hence similar to \Cref{lem:small-circles-white-grid-cells} we state the following lemma for $d$-dimensional case also using \Cref{lem:small-hypersphere-grid-cells}, \Cref{lem:gray-circles-d}, \Cref{lem:white-circles-d}.
	\begin{lem}
		\label{lem:small-circles-white-grid-cells-d}
		There
		is a set $\C'_S \subseteq \C^*_S$ of small hyperspheres with
		$p(\C'_S)\geqslant (1-\eps) p(\C^*_S)$
		such that there is a packing for $\C'_S$ using the grid cells in $\G_w$ only.
	\end{lem}
	We extend \Cref{lem:grid-resource-augmentation} for the $d$-dimensional case.
	\begin{lem} \label{lem:grid-resource-augmentation-d}
		There is a set of small hyperspheres $\C''_{S}\subseteq\C'_{S}$ such that $p(\C''_{S})\geqslant(1-\eps)p(\C'_{S})$
		and it is possible to place the hyperspheres in $\C''_{S}$ non-overlappingly
		inside $|\G_{w}|$ $d$-dimensional knapsacks of size $(1-\eps)\epsc \times\dots \times(1-\eps)\epsc$
		each. \end{lem}
	\begin{proof}
			Consider a $d$-dimensional knapsack in $\G_{w}$ of side length $\epsc$.
		By removing  all circles intersected by a random strip of width $\eps*\epsc$ in all the d directions, we incur a loss of at most $d(d r/\epsc + \eps)$ fraction of optimal profit. As $r\le \epss$, we incur a loss of at most $O(\eps)$ fraction of profit as $\epss = \epsc^2 = \epsl^{12d}$.
		
	\end{proof}
	We further extend \Cref{lem:structured-packing} to $d$-dimensional case using \Cref{lem:grid-resource-augmentation-d}
	\begin{lemma}\label{lem:structured-packing-d}
		In polynomial time, we can compute a set of grid cells $\G_w$ such that no grid cell in $\G_w$ intersects with any
		hypersphere $C_i \in\C_{L}^{*}$ for any legal placement of $C_i$. Moreover, there is a set of small circles $\C_S \subseteq \C_{S}^{*}$ such that $w(\C_{S}) \geqslant (1-\eps)w(\C_{S}^{*})$ and
		the circles in $\C_S$ can be packed non-overlappingly inside $|\G_w|$ grid cells of size $(1-\eps) \epsc \times\dots\times(1-\eps) \epsc$ each.
	\end{lemma}
	%Using it, we compute an approximation to the set $\C_S$ via the following result from \cite{MiyazawaWAOA}.
		Using it, we compute an approximation to the set $\C_S$ via an extension of our result from \Cref{thm:fat-ra} to $d$-dimensions and setting fatness $f$ to 1 for spheres.
	
	
	We pack the computed hyperspheres into our grid cells $\G_w$, denote them by $\C'_S$. In particular, they do not intersect any of the
	large hyperspheres in $\C_{L}^{*}$ in any legal placement of them. Our solution (corresponding to the considered guesses) consists of $\C_{L}^{*}\cup \C'_S$.

In order to further improve the precision of the large hyperspheres, we replicate techniques from \Cref{subsec:Improve_Large} which completes the proof of \Cref{thm:d-dim-ptas}


\subsection{Proof of Lemma \ref{lem:small-circles-white-grid-cells-1}}
%
% \begin{restatable}{lem}{smallcircleswhitegridcellslemmaapx}
% 	\label{lem:small-circles-white-grid-cells-1}
% 	There is a set $\C'_S \subseteq \C^*_S$ of small circles with $p(\C'_S)\geqslant (1-\eps) p(\C^*_S)$ such that there is a packing for $\C'_S$ using the grid cells in $\G_w$ only.
% \end{restatable}
% \begin{proof}
	We delete all circles in the $\eps$ fraction of white cells with the smallest total
	weight among all white cells, incurring an $\eps$ fraction loss in the weight.
	This makes $\eps \epsl^2/4$ space available for packing circles in the gray cells and $\C_{cut}$.
	Now, total volume of circles in the gray cells and $\C_{cut}$ is at most  $\eps \epsl^2/5 + \eps \epsl^2/64 \leqslant \eps \epsl^2/4$

	Recall that the radius of each
	small circle is at most $\epss$, which is at least by a factor
	$1/\eps$ smaller than the size of each grid cell (which is $\epsc \times\epsc$).
	Therefore, with a shifting argument we can show that from each grid
	cell $G_{\ell,\ell'}\in\G$ we can delete small circles from $\C'_S$ contained in
	$G_{\ell,\ell'}$ whose total profit is only an $O(\eps)$-fraction
	of the overall profit of those circles, such
	that the remaining circles in $G_{\ell,\ell'}$ fit even inside a smaller
	grid cell of size $(1-\eps)\epsc \times(1-\eps)\epsc$.
	If we apply this operation to each grid cell in $\G_{w}$, the remaining
	circles fit non-overlappingly into $|\G_{w}|$ (small) knapsacks of
	size $(1-\eps)\epsc \times(1-\eps)\epsc$
	each.
% \end{proof}

\subsection{Proof of Lemma \ref{lem:grid-resource-augmentation-1}}
%
% \begin{restatable}{lem}{gridresourceaugmentationlemmaapx}
% 	\label{lem:grid-resource-augmentation-1}
% 	There is a set of small circles $\C''_{S}\subseteq\C'_{S}$ such that $w(\C''_{S})\ge(1-\eps)w(\C'_{S})$ and it is possible to place the circles in $\C''_{\sml}$ non-overlappingly inside $|\G_{w}|$ square knapsacks of size $(1-\eps)\epsc \times(1-\eps)\epsc$ each.
% \end{restatable}
% \begin{proof}
	Consider a square knapsack in $\G_{w}$ of side length $\epsc$.
	By removing  all circles intersected by a random strip of width $\eps*\epsc$ in both directions, we incur a loss of at most $2(2 r/\epsc + \eps)$ fraction of optimal profit. As $r\le \epss$, we incur a loss of at most $O(\eps)$ fraction of profit as $\epss = \epsc^2 = \epsl^{24}$.
% \end{proof}




\section{Omitted Proofs from \Cref{sec:polygon}}

\subsection{Proof of \Cref{lem:create-gap-polygons}}
\begin{proof}We set $\rho_k=(\rho_{k-1})^{24}$ in \Cref{lem:shifting} and immediately get the required result.
%	\arir{Add in the appendix}
\end{proof}

\subsection{Proof of \Cref{lem:structured-packing-polygon}}

\begin{lem}
	\label{lem: cut-polygon}
	Let $\mathcal{P}_{cut}\subseteq \P_{S}^{*}$ be the set of all small polygons in $\P_{S}^{*}$ that intersect more than one grid cell. We have that $\area(\mathcal{P}_{cut}) \le 8 f \epss/\epsc \le f \eps \epsl^2/64$.
\end{lem}

\begin{proof}
	For each horizontal (resp. vertical) gridline $\ell$, each $P \in \mathcal{P}_{cut}$ must lie in a strip of height (resp. width) $4 r^{out} \le 4f r^{in} \le 4f \epss$ and width (resp. height) 1. In total, there are $2/\epsc$ gridlines.
	Thus, $\area(\mathcal{P}_{cut}) \le 8 f\epss/\epsc = 8 f \epsl^{12}  \le  f \eps \epsl^2/64$. The last inequality follows from the fact that $\epsl \le \eps \le 1/2$.
\end{proof}

We will repack polygons from $\mathcal{P}_{cut}$ later. Now we again partition cells into gray, white, and black as before.

\begin{defn} Let $G_{\ell,\ell'}\in\G$ for some $\ell,\ell'\in\{0,1,...,1/\epsc-1\}$.
	The cell $G_{\ell,\ell'}$ is
	\begin{itemize}
		\item \emph{white} if $G_{\ell,\ell'}$ does not intersect with any polygon
		$P_{i}\in\C_{L}^{*}$,
		\item \emph{black} if $G_{\ell,\ell'}$ is contained in some polygon $P_{i}\in\P_{L}^{*}$,
		\item \emph{gray }if $G_{\ell,\ell'}$ is neither white nor black.
	\end{itemize}
\end{defn} 


\begin{lem} \label{lem:gray-circles-polygon}The total area of gray
	cells $\area(\G_{g})$ is at most  $80 f \epsc/ \epsl \le f \eps \epsl^2/3$. We can compute $\G_g$ in polynomial time.
\end{lem} 
\begin{proof}
	The perimeter of a single large convex polygon $P_i$ is upper bounded by $2 \pi r^{out} \le 2 f \pi r^{in}$. Let us divide the perimeter of $P_i$ into at most $\lceil\frac{2 f \pi r^{in}}{\epsc}\rceil$ pieces of length $\epsc$.
	One such piece intersects at most $9$ grid cells, so the total number of grey cells created by $P_i$ is upper bounded by $9 \epsc^2 \lceil\frac{2 f \pi r^{in}}{\epsc}\rceil$, which is roughly  $\le 20f\pi r^{in}\epsc$. 
	
	From the proof of \Cref{lem:gray-circles} we know that all cells inside the circle with a radius of $r^{in}- 3\epsc$ are black. Hence we get that the fraction \[
	\frac{\area(\G_{g, P_L})}{\area(\G_{b, P_L})} \leq \frac{20 f \epsl \epsc}{(\epsl - 3 \epsc)^2} \leq \frac{80 f \epsc}{\epsl}
	\]
	The last inequality follows from the fact that $\epsc \leq \frac{1}{6} \epsl$ or $\eps \leq 1/6$. 
	The total area of all black cells is at most one so we get that the total area of all gray cells is at most $\frac{80 f \epsc}{\epsl} \le 80 f \epsl^{11} \le f \eps \epsl^2 / 3$.
\end{proof}


As before, we now show that the number of white cells is much larger than the number of gray cells.

\begin{lem} \label{lem:white-polygons}
	The total area of white grid cells $\area(\G_{w})$ is at least $\left ( \frac{16 \pi^2 {\sin(\alpha)}^2{\cos(\alpha)}^2}{q^2 t^2 (\sin(\alpha)+\cos(\alpha))^2} \right )\cdot \epsl^2$. We can compute $\G_w$ in polynomial time.
\end{lem}
\begin{proof}
	Consider a corner (w.l.o.g., left bottom corner) $v_{lb}$ of the knapsack. Let  $S_w$ be a square region of side length $\left ( \frac{2 \pi {\sin(\alpha)}{\cos(\alpha)}}{q t (\sin(\alpha)+\cos(\alpha))} \right ) \epsl$ such that $S_w$ is contained in the knapsack and shares $v_{lb}$. $S_w$ lies inside the bin for small enough values of $\epsl$ and in turn $\eps$.
	We will show that no large polygons intersect $S_w$ and thus all grid cells in $S_w$ are white.
	First note that since the polygon is $t$-regular and has at most $q$ sides, 
	$2\pi r_{in} \le q s_{max} \le q t s_{min}$, where $s_{max}, s_{min}$ denote the maximum and minimum length of the sides of a large polygon.
	Now since $r_{in} \ge \epsl$ for large polygons, we have $s_{min} \ge \frac{2\pi \epsl}{q t}$.
	
	Now, consider the case, when one of the shortest sides of a large polygon makes an angle $\alpha$, with the side of the knapsack bin, 
	it is easy to see the square $S_w$ is not intersected. For brevity, we do not repeat the arguments. 
	
	
	%Now, it is easy to see geometrically that even in the worst case when one of the shortest sides of a large polygon makes an angle $\alpha$, with the side of the knapsack bin, the square $S_w$ is not intersected.
	
	We can now argue this analogously for all the corners of the knapsack and the lemma is proved. 
%	\arir{move to appendix and add a figure.}
\end{proof}

\begin{lem} \label{lem:small-circles-white-grid-cells}There
	is a set $\P'_S \subseteq \P^*_S$ of small polygons with
	$p(\P'_S)\ge (1-O(\eps)) p(\P^*_S)$
	such that there is a packing for $\P'_S$ using the grid cells in $\G_w$ only.
\end{lem}
\begin{proof}
	We delete all polygons in the $\left( \frac{q^2 t^2 (\sin(\alpha)+\cos(\alpha))^2}{32 \pi^2 {\sin(\alpha)}^2{\cos(\alpha)}^2}\right)\eps$ fraction of white cells with the smallest total
	weight among all white cells, incurring an $\left( \frac{q^2 t^2 (\sin(\alpha)+\cos(\alpha))^2}{32 \pi^2 {\sin(\alpha)}^2{\cos(\alpha)}^2}\right) \eps$ fraction loss in the weight. The fraction of polygons we delete has to be smaller than 1, which is true for small enough $\eps$.
	This makes $\eps \epsl^2 /2$ space available for packing polygons in the gray cells and $\P_{cut}$. 
	Now, total volume of polygons in the gray cells and $\P_{cut}$ is at most  $f \eps \epsl^2/3 + f \eps \epsl^2/64 \le f \eps \epsl^2 /2$.
\end{proof}

\begin{lem} \label{lem:grid-resource-augmentation}There is a set
	of small polygons $\P''_{S}\subseteq\P'_{S}$ such that $w(\P''_{S})\ge(1-\eps)w(\P'_{S})$
	and it is possible to place the polygons in $\P''_{\sml}$ non-overlappingly
	inside $|\G_{w}|$ square knapsacks of size $(1-\eps)\epsc \times(1-\eps)\epsc$
	each. \end{lem}
\begin{proof}
	Consider a square knapsack in $\G_{w}$ of side length $\epsc$.
	Remove  all polygons intersected by a random strip of width $\eps$ for both directions, we incur at most a $(1-O(\eps))$-factor loss in the weight.
\end{proof}
This completes the proof of Lemma~\ref{lem:structured-packing-polygon} with $\P_{S}:= \P''_{S}$.

%\subsection{Proof of \Cref{thm:polytope}}
%We recall all notations and techniques from \Cref{sec:polygon}. We first use the shifting technique from \Cref{lem:shifting} on the $r_{in}$ of the polytope items $P$ to remove the set of medium items given an $\eps$. We set \(f(x)=x^{12d}\) in \Cref{lem:shifting} and \(\eps^{j}=(\eps^{j-1})^{12d}\) in  \Cref{lem:create-gap}.
%Then we adapt the linear program as described in \Cref{sec:polygon} to pack a guessed set of large polytope items.
%To pack the set of small polytopes, we use the following two lemmas.
%
%\begin{lemma}
%	If all given polytope items are $(f,q,t,\beta)$-well-behaved and given $\eps$ is a small enough constant then
%	\begin{itemize}
%		\item in polynomial time we can compute a set of grid cells $\G_w$ such that no grid cell in $\G_w$ intersects with any
%		polytope $P_i \in\P_{L}^{*}$,
%		\item there is a set of small polytope items $\P_S \subseteq \P_{S}^{*}$ such that $w(\P_{S}) \ge (1-O(\eps))w(\P_{S}^{*})$ for the optimal packing of the large polytope items, and
%		\item the polytope items in $\P_S$ can be packed non-overlappingly inside $|\G_w|$ grid cells that have size
%		\mbox{$(1-\eps) \epsc \times ... \times (1-\eps) \epsc$} each.
%	\end{itemize}
%\end{lemma}
%
%\begin{proof}
%	Recalling the analysis and definitions from the \Cref{sec:spheres} on $d$-dimensional spheres and \Cref{sec:polygon} on polygons, we have $a(P_{cut}) \leq 4df\epss/\epsc \leq df\epsl^d/2^{5d-3}$. 
%	
%	To calculate the total volume of gray grid cells $a(G_{gray})$, we first note that the surface area of the polytope item is bounded by the surface area of hypersphere of radius $r_{out}= f'\cdot r_{in}$. The number of cells the polytope item intersects is at most $9d$ times the number of cells the outer hypersphere intersects as the polytope is convex. From the \Cref{lem:gray-circles-d}, the number of gray cells that the hypersphere intersects is at most \(\dfrac{f^d(d+1)(3^d-1)\eps\epsl^d}{2^{5d-3}}\). Hence we get $a(G_{gray}) \leq \dfrac{9f^d d(d+1)(3^d-1)\eps\epsl^d}{2^{5d-3}}$.
%	
%	Next, we try and find a minimum bound on the volume of white grid cells using an empty space that cannot be packed in the corner by a \textit{large} polytope item. We are guaranteed that an empty space will be left in the corner as all of the $k$-hedral angles are guarenteed to \ag{be} larger than $\pi/2$. Now, we know that for a large polytope item, $r_{in}> \epsl$. Since there are at most $q$ sides, the maximum ratio of lengths between any two sides is $t^q$. We get that the empty space at the corner will be at least $O_{\phi, \beta, t,q, d}(1)\cdot 1/\epsc^d \le O_{\phi, \beta, t,q, d}(1) \cdot \eps \epsl^d$.
%	
%	Using the randomized strip argument as in 
%	\Cref{lem:grid-resource-augmentation-d}, using the same procedure again as in \Cref{sec:polygon}, we are done.
%\end{proof}
%
%\begin{lemma}
%	Given a set of $m$ knapsacks of size $(1-\eps) \epsc \times ... \times (1-\eps) \epsc$
%	each and a set of $(f,q,t,\beta)$-well-behaved polytope items $\bar{\P}$, each of which can be enclosed in a cell of size $(1-\eps) \epsc \times ... \times (1-\eps) \epsc$. 
%	Then in polynomial time we can compute a set of polytope items $\bar{\P}'\subseteq\bar{\P}$ and
%	a non-overlapping placement of the polytopes in $\bar{\P}'$ inside $m$
%	knapsacks of size $\epsc \times ...\times \epsc $ each, such
%	that $w(\bar{\P}')\ge(1-\eps)w(\bar{\P}^{*})$ for any set of
%	polytope items $\bar{\P}^{*}\subseteq\bar{\P}$ that can be placed non-overlappingly
%	in the given $m$ knapsacks of size $(1-\eps)\epsc\times(1-\eps)\epsc$ each. 
%\end{lemma}
%
%\begin{proof}
%	Most of the steps to prove this theorem follow along the same lines as the proof of \Cref{thm:fat-ra}. We describe the changes that need to be made. 
%	
%	In \Cref{lem:grid-resource-augmentation}, the object $P$ overlaps with at most $10d [(f r_{in})^{d-1}/d^d {\delta_{cell}}^{d-1}] \delta_{cell}^{d} \leq 10 (f r_{in})^{d-1} \delta_{cell} $ and we can choose $\delta_{cell} \leq \eps \delta_{large}/ 80 f d$ to have a small fraction of gray cells. 
%	
%	Other than this we will need to redefine $\delta_{c,i} = \delta_{cell} (\delta_{c,(i-1)})^{d+4}$, keeping the other recurrences and values the same. This change was needed to bound the total shift at the end of the proof of \Cref{lem:fatdiscrete}.
%	
%	Everything else involved in extending remains the same and  was independent of dimension.
%\end{proof}
%
%Using the above two lemmas and using them in the same fashion as before, we can get a PTAS for the problem.

%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\subsubsection{Proof of Theorem~\ref{lem:resource-augmentation-polygon}}\label{app:thm-resource-augmentation-polygon}
In this section, we in fact, prove a stronger claim (Theorem \ref{thm:fat-ra}) than Theorem~\ref{lem:resource-augmentation-polygon} as we claim we can pack in a bin augmented in only one dimension.
Let $P_i$ be a two-dimensional polygon and let $r_{i}^{\mathrm{out}}(P_i)$ and $r_{i}^{\mathrm{in}}(P_i)$ be
the radius of the smallest circle containing $P_{i}$ and the radius
of the largest circle contained in $P_i$, respectively. 
We will drop $P_i$ when it is clear from the context. 
We say that $P_i$ is $f$\emph{-fat} if  $r_{i}^{\mathrm{out}}/r_{i}^{\mathrm{in}}\le f$
for some value $f$.

\begin{theorem}
	\label{thm:fat-ra}
	Let $f>0$ and $\eps>0$. Given a set of $f$-fat convex objects, there exists a polynomial time algorithm that can pack a subset of them with a total weight of $\profit(\OPT)$ into a knapsack $[0, 1+\eps] \times [0, 1]$, where  $\profit(\OPT)$ is the optimal profit that can be packed into a knapsack $[0, 1] \times [0, 1]$.
\end{theorem}

Now we prove \Cref{thm:fat-ra}. 
Given a packing of a set of $f$-fat objects $\mathcal{P}=\{P_1, P_2, \dots, P_n\}$ in our knapsack $K=[0, 1] \times [0, 1]$, we want to show that there is also a structured packing of these objects, defined via a discrete grid.
Let $\dc>0$ be a constant to be defined later such that $1/\dc \in \mathbb{N}$. We place a grid inside $K$ such that each grid cell has an edge length of $\dc$. Let $\mathcal{G}$ denote set of all resulting grid cells. Assume first that our polygons in $\mathcal{P}$ are all $\dl$-large (i.e., $r^{in} \ge \dl$) for some given constant $\dl>0$. We say that our given packing for $\mathcal{P}$ is {\em discretized} if
there is a partition of $\mathcal{G}$ into sets $\{\mathcal{G}_{P_1}, \mathcal{G}_{P_2}, \dots, \mathcal{G}_{P_n}\}$ such that for each
$i$, we have that $P_i$ is contained in the union of the cells in $\mathcal{G}_{P_i}$.
%
%
% Given a packing of a set of $n$ $\sigma$-fat objects $\mathcal{P}=\{P_1, P_2, \dots, P_n\}$, we say the packing is {\em discretized} if the packing can be divided into disjoint
% sets $\{\mathcal{G}_{P_1}, \mathcal{G}_{P_2}, \dots, \mathcal{G}_{P_n}\}$, such that each $\mathcal{G}_{P_i}$ contains only $P_i$ and none of the other objects in $\mathcal{P}$ overlap with $\mathcal{G}_{P_i}$ and $\mathcal{G}_{P_i}$ is union of contiguous grid cells of length at least  $\dc r_{i}^{\mathrm{in}}(P_i)$ for some given constant $\dc$.
% And we call $P_i$ is discretized to $\mathcal{G}_{P_i}$.
We show that for an appropriate choice of $\dc$, there is a discretized packing for $\mathcal{P}$ if we can increase the size of our knapsack by a factor of $1+\delta$ in one dimension.

\begin{lemma}
	\label{lem:fatdisc}
	For each $f>1$, $\eps>0$, and $\dl>0$, there is a value $\dc>0$ such that for any set of $\dl$-large $f$-fat objects $\mathcal{P}$
	that can be placed non-overlappingly inside a knapsack $K=[0, 1] \times [0, 1]$, there is a discretized packing for $\mathcal{P}$ inside a knapsack of size $[0, 1+\eps] \times [0, 1]$.
	% according
	% Given a placement of a fat object $P$ with $r_{in} \ge \dl N$ in a bounded box $[0,N]^2$, where $N \in \mathbb{Q}$, we can discretize it to $\mathcal{G}_P$, a union of grid cells of length at least  $\dc \cdot r_{i}^{\mathrm{in}}(P)$ such that $(\area(\mathcal{G}_P)-\area(P))/\area(P) \le  \eps$.
\end{lemma}
\begin{proof}
	By the classical Barbier's theorem, we know  the perimeter of a convex set $P$ is at most $\pi \cdot \text{diameter}(P) \le 2\pi r^{out} \le 2\pi \sigma r^{in}$.
	
	Now we can break the perimeter into  $\lceil (2\pi f r^{in)}/ (\dc)  \rceil$ curved segments of length at most $\dc$. Each such segment can at most intersect with 9 grid cells.
	
	Hence, total area of the grid cells with which the perimeter of $P$ overlaps is at most $9 \lceil (2\pi f r^{in)}/ (\dc)  \rceil \times (\dc )^2 \leq 20\pi f r^{in} \dc$.
	Therefore,  $(\area(\mathcal{G}_P)-\area(P))/\area(P) \le  \frac{20\pi f r^{in} \dc }{\pi(r^{in}-2\dc )^2} \le  \frac{20\pi f \dl  \dc }{\pi(\dl  - 2\dc )^2}
	\le  \frac{20 f \dl \dc}{(\dl-2 \dc)^2}  \le \eps$, by choosing  $\dc \le \eps \dl/ 80 f$.
\end{proof}

Next, we argue that there is also a structured packing for fat objects that are not necessarily all large.
Let $\dl,\dc,\ds>0$ be constants (dependent on $\eps$, another constant) to be defined later.
% $\delta \ge \dl \ge  \dc \ge \ds$ be three constants that we will choose later.
We define $\delta_{c,0}=1$ and $\delta_{s,0}=1$, $\delta_{l,i}=\dl {\delta_{c,{(i-1)}}}, \delta_{s,i}=\ds \delta_{c,{(i-1)}}$, and $\delta_{c,i}=\dc \delta_{c,{(i-1)}}^6$.
We call $L_i$ to be the items with $r^{out} \in (\delta_{l,i}, \delta_{s,{i-1}}]$, and $M_i$ to be the items with $r^{in} \in (\delta_{s,i}, \delta_{l,{i}}]$.
With standard shifting argument, we set values for $\dl = \eps, \ds = \eps^3$
so that the total volume of the items in any set $M_i$ is at most $\eps/10 f^2$ (assuming $\eps<1/10f^2$).

We generalize now our notion of discretized packings to arbitrary  $f$-fat objects (not necessarily large). Let $\mathcal{P}$ be a set of $f$-fat objects. We place a hierarchical grid. We define that the whole knapsack $K$ is one grid cell of level 0 of side length $\delta_{c,0}=1$. Recursively, each grid cell of some level $\ell$ is partitioned into $\delta_{c,\ell+1}^2$ grid cells of level $\ell+1$ with side length $\delta_{c,\ell+1}$ each. We say that our packing of $\mathcal{P}$ is \emph{discretized} if
\begin{itemize}
	\item for set set $L_i$ and for each object $P\in \mathcal{P}\cap L_i$ there is a set of $O(1/\delta_{c,i}^2)$ grid cells $\mathcal{G}_P$ of level $i$ such that $P$ is contained in $\mathcal{G}_P$, and there is a single grid cell of level $i-1$ which contains all grid cells in $\mathcal{G}_P$, and
	\item for any two objects $P,P'\in \mathcal{P}$ (not necessarily of the same level) the grid cells in $\mathcal{G}_P$ and $\mathcal{G}_P'$ are pairwise non-overlapping.
\end{itemize}

We show that by increasing the size of our knapsack by a factor of $1+\delta$, there is a discretized packing for all objects in the sets $L_i$. We will pack the items in the sets $M_i$ later separately. This will be easy since their total area is very small.

% for any  non-increasing function $f,g$ such that $\dc=g(\dl), \ds=f(\dc)=fg(\dl)$ and total volume of items in $M_i$ is at most $\eps/10 \sigma^2$ and profit of items in $M_i$ is at most $\eps \profit(\mathcal{P})$.
% Note that, as the data is polynomially bounded, number of classes $L_i$ is at most $O(\log n)$.
% Now we show that given any packing for fat objects in $[0, 1] \times [0, 1]$, we can obtain a  {\em discretized packing} in $[0, 1+\delta] \times [0, 1]$ knapsack and a later we will employ a DP to find a packing with at least the same profit.

\begin{lemma}
	\label{lem:fatdiscrete}
	For each $f>1$ and $\eps>0$, there are values $\dl, \ds, \dc>0$ such that for any set of $f$-fat objects $\mathcal{P}$
	that can be placed non-overlappingly inside a knapsack $K=[0, 1] \times [0, 1]$, there is a discretized packing for $\mathcal{P}$ inside a knapsack of size $[0, 1+\eps] \times [0, 1]$.
	% according
	% Given a placement of a fat object $P$ with $r_{in} \ge \dl N$ in a bounded box $[0,N]^2$, where $N \in \mathbb{Q}$, we can discretize it to $\mathcal{G}_P$, a union of grid cells of length at least  $\dc \cdot r_{i}^{\mathrm{in}}(P)$ such that $(\area(\mathcal{G}_P)-\area(P))/\area(P) \le  \eps$.
\end{lemma}
\begin{proof}
	Let $\eps \ge \dl= \eps \ge  \dc=\eps^2 \ge \ds=\eps^3$ be three constants.
	We define $\delta_{c,0}=1$ and $\delta_{s,0}=1$, $\delta_{l,i}=\dl \delta_{c,{(i-1)}}, \delta_{s,i}=\ds \delta_{c,{(i-1)}}$, and $\delta_{c,i}=\dc \delta_{c,{(i-1)}}^6$.
	We call $L_i$ to be the items with $r^{out} \in (\eps_{l,i}, \eps_{s,{i-1}}]$, and $M_i$ to be the items with $r^{in} \in (\eps_{l,i}, \eps_{s_{i}}]$.
	With standard shifting argument, we find that total area of items in $M_i$ is at most $\eps/10 f^2$ (assuming $\eps<1/10f^2$) and weight of items in $M_i$ is at most $\eps \profit(\mathcal{P})$.
	Note that, as the data is polynomially bounded, number of classes $L_i$ is at most $n^{O(1)}$. 
	
	Starting with $\mathcal{P}$, we will do a sequence of translations so that the final packing becomes discretized. 
	Let us have a packing in the $i$th level in $[x  \delta_{c,i}, (x+1) \delta_{c,i}] \times [y\delta_{c,i}, ((y+1)\delta_{c,i}]$ for some $x,y \in \{0, 1, \dots, \delta_{c,i}-1\}$. 
	
	Now consider gridcells of length $\delta_{c,i}$. Items in $L_i$ are large compared to the gridcells. 
	From \Cref{lem:fatdisc},  we can ensure that we can remove a small area compared to the packed area to make the packing discretized.
	We also remove all items from group $L_{i+2}$ that intersects the gridlines  (defined by $\delta_{c,i}$ width). Using a random shift argument, we can claim that they are cut by the gridlines with very small probability and thus the total area of such cut items is again very small. 
	These three set of removed items, corresponding to $\cup_i M_i$, removed items due to discretization, and removed items due to intersection with gridlines, totally constitute only $O(\eps)$ volume. 
	Choosing appropriate constants $\dc,\dl,\ds$, we can ensure that these removed items are packed in a discretized way in some $\eps/2$ width-strip in the augmented region.
	
	Finally, we use the augmentation region to translate the packing so that the discretized regions corresponding to two objets in $L_i$ don't overlap. ´
	Let $A_i$ be the total area of fat objects from $L_i$ that were discretized.
	Then, on $i$'th level, at most $A_i/(\pi \delta_{l,i}^2)$ fat objects were discretized and each such object can overlap at most $10 f^2/\dl^2$ other items from $L_i$.
	So, total shift needed $\le \sum_i (A_i/(\pi \delta_{l,i}^2)) \cdot  10 f^2/\dl^2 \cdot  \delta_{c,i} \le 40f \delta_{c,i}/(\delta_{l,i}^2 \dl^2) \le 40f \dc \delta_{c,(i-1)}^4/\dl^4 \le 40f (\eps^2)^4/eps^4 \le 40f\eps^4$. 
	We can ensure that the total shift is at most $\eps/2$, if we choose $\eps<1/10f^2$ as already assumed.
	
	This completes the proof of this lemma.
\end{proof}

Now we describe a dynamic program that finds a discretized packing for our items in the sets $L_i$.
% Note that we can guess $O_{1/\eps}(1)$ we can guess $\dl, \ds, \dc$.
We introduce a DP-cell
% Each cell in our DP-For the correct guess, let the DP-cell is
$DP[i, m]$ for each combination of a value $i$ which is the index of a set $L_i$ and a value $m\in \{1,...,n\}$. This cell corresponds to the subproblem
of packing all items in $L_i,L_{i+1},L_{i+2},\dots.$ via a discretized packing into $m$ knapsacks with side length $\delta_{c,(i-1)}$  each. Observe that we can pack only constantly many items from $L_i$ into each of these $m$ knapsacks. Thus, there are only constantly many options how the corresponding set $\mathcal{G}_{P}$ of such an object $P\in L_i$ can look like. We say that a \emph{configuration} is a combination of constantly many of these possible sets $\mathcal{G}_{P}$ whose grid cells are pair-wise non-overlapping. Thus, there are only constantly many configurations. Denote by $M$ their total number. We guess in time $m^{O(M)}\le n^{O(M)}$ how many knapsacks have each of the (at most $M$) configurations. Then, we assign the items in $L_i$ into the knapsacks according to this guess. We can do this with a simple bipartite matching since for each object $P' \in L_i$ and each possible set $\mathcal{G}_{P}$ we can check easily whether $P'$ fits into $\mathcal{G}_{P}$. Our guess yields a number $m'$ of empty knapsacks of the next level $i+1$ into which we need to pack the items in $L_{i+1},L_{i+2},\dots$. We assign these items according to the solution in the DP-cell $DP[i+1, m']$.
As, there are at most $n$ items, note that $m'$ remains at most $n$. Note that, as the data is polynomially bounded, number of classes $L_i$ is also at most $n^{O(1)}$.  Thus, the DP runs in $n^{O(M)}$ time. 

We can additionally pack the medium objects from the sets $M_i$ separately in a strip of the form $[0,1] \times [1, 1+O(\eps)]$ by a volume argument. For example, it is sufficient to replace each of these objects by the smallest rectangle that contains it (which increases its area only by a constant factor since each item is fat). The resulting rectangles can then be placed non-overlappingly with the $\mathtt{NFDH}$ algorithm explained in \cite{NFDH}.
This completes the proof of \Cref{thm:fat-ra}.

\end{comment}
%%%%%%%%%
%%%%%%%%%%%

%%%%%%%%%
%%%%%%%%%%%
\begin{comment}
\subsection{Proofs from \Cref{sec:rational}: Spheres with only rational coordiantes}
In the $\mathsf{d-CSK}$ problem, we are given a set $\mathcal{C}$ of weighted $d$-dimensional hyperspheres, and we wish to pack maximum profit into a unit bin.
For a constant $\eps>0$, we first get a packing $P$ into the augmented bin of size \((1+\eps) \times ... \times 1\).


As discussed earlier, the geometric knapsack problem involving circles, or $d$-dimensional hyperspheres, lacks clarity regarding the existence of an optimal or $(1+\eps)$-approximate solution that utilizes solely rational coordinates. In this work, we establish that for each dimension $d\leqslant8$, there exists a polynomial-time $(2+\eps)$-approximation algorithm capable of producing a solution exclusively with rational coordinates, encoded with a polynomial number of bits. This result implies the guaranteed existence of solutions with rational coordinates, consistently at most a factor of $2+\eps$ worse than the optimal solution with arbitrary coordinates. Moreover, for arbitrary dimensions, we present a $3$-approximation algorithm that utilizes exclusively rational coordinates, with the representation requiring a polynomially bounded number of bits.

%We propose a $3$-approximation algorithm that works for all dimensions and improve upon it to give a $(2+\eps)$-approximation algorithm that works only for dimensions $d\leqslant 8$.

\subsubsection{Augmented Optimal Packing}

Let $\OPT$ be an optimal solution, $\C_{\OPT}$ be the spheres in $\OPT$, and $w(\OPT)$ be the optimal weight.

%\begin{restatable}{theorem}{extendedwoawabs}
\begin{theorem}
	\label{extended-wowa}
	Let $\mathcal{C}$ be an instance of the $\mathsf{d-CSK}$ problem and \(\eps \geqslant 0\) be a small enough constant. There is a polynomial time algorithm that finds a packing $P$ of a subset \(\mathcal{C}^'\subseteq \mathcal{C}\) in an augmented knapsack of size \((1+\eps) \times \cdots \times 1\) such that \(p(\mathcal{C}^')\geqslant w(\OPT) \), where $\OPT$ is the optimal solution.
	\end{theorem}
%\end{restatable}
\begin{proof}
	
	We use the shifting strategy mentioned in section \Cref{lem:shifting} with $\rho_{k,1}= \eps^k$ to get a set of hyperspheres $\mathcal{C}_M$ with a total weight less than $\eps \cdot w(\OPT)$ and radius between $\eps^{\tau_1-1}$ and $\eps^{\tau_1}$ for some $\tau_1<1/\eps$. Now, we use the shifting strategy again on the set $\mathcal{C}_M$ but for volume instead of weight. With $\rho_{k,2} =\eps^{\frac{k\tau_1 - 1}{k}}$, there is a $\tau_2 \leqslant 1/\eps$ as the total volume of $\mathcal{C}_M$ is at most 1, such that we can get a set of hyperspheres $\mathcal{C}_{removed}$ such that it has a total profit less than $\eps \cdot w(\OPT)$, total volume less than $\eps$, and all radii between $\rho_{\tau_2-1, 2}$ and $\rho_{\tau_2, 2}$. 
	
	Using the algorithm provided in \cite{MiyazawaWAOA}, for a suitable constant $\eps'$, such that the set of medium hyperspheres described in \Cref{lem:shifting} removed is the same as the $\mathcal{C}_{removed}$ above, we get a packing of $w(\OPT) - w(\mathcal{C}_{removed})$ total weight in a bin of size \((1+\eps') \times \cdots \times 1\). Now, notice that $\mathcal{C}_{removed}$ can be packed into a unit slab of width $O(\eps)$ using the $\mathtt{NFDH}$ algorithm explained in \cite{NFDH}. Join this slab to our already augmented bin to get a further augmentation but a packing of $w(\OPT)$. Choose an $\eps''= \eps+\eps'$ to get our result.
\end{proof}
\subsubsection{$3$-approximation algorithm for all dimensions $d$} \label{sec:appendix-3-apx}

Using \Cref{extended-wowa}, we get a packing $P$ in the augmented hypercube of dimensions $(1+\eps)\times 1 ...\times 1$ such that the total packed profit is at least $w(\OPT)$.

Call two $\eps$-augmenting planes $\ell$ and $\ell'$ which are perpendicular to the augmented side of the hypercube of length $1+\eps$ and are at a distance of $\eps$ from the left face and right face respectively. Let us define three types of hyperspheres in the packing $P$ obtained above in the augmented hypercube as shown in \Cref{fig:partition-img-3bins}. Define \textit{type 1 hyperspheres} to be the hyperspheres in $P$ which are completely inside the $(1-\eps)\times 1 \times ... \times 1$ $d$-dimensional slab to the left of $\ell$ and to the right of $\ell'$, \textit{type 2 hyperspheres} to be the hyperspheres in $P$ which intersect $\ell$, \textit{type 2' hyperspheres} to be the hyperspheres in $P$ which intersect $\ell'$, and finally \textit{type 3 and 3' hyperspheres} to be the hyperspheres in $P$ which are completely contained inside the `$\eps$-slab' of dimensions $\eps\times 1 \times ... \times 1$ to the right of $\ell$ and left of $\ell'$, respectively. We now prove that for small values of $\eps$, there can be at most one \textit{huge} hypersphere that intersects both $\ell$ and $\ell'$. Since the distance between $\ell$ and $\ell'$ is $1-\eps$, a \textit{huge} hypersphere must have a diameter of at least $1-\eps$ to intersect both $\ell,\ell'$.

%\begin{restatable}{lemma}{nextradabs}
\begin{lemma}
	\label{nextrad}
	If a huge hypersphere i.e., a hypersphere with a diameter greater than or equal to $1-\eps$ is packed in the augmented bin of dimensions $(1+\eps)\times 1 \times \ldots \times 1$, then the radius of the second biggest hypersphere is at most $\frac{1}{2}+\frac{1}{d-1}+\eps\left(\frac{1}{2} + \frac{2}{d-1}\right) -\sqrt{\frac{(1+\eps)^2}{(d-1)^2}+\frac{1-\eps^2}{d-1}}$.
	\end{lemma}
%\end{restatable}
\begin{proof}
	The radius of the next hypersphere will be the biggest when the the diameter of the \textit{huge} sphere is exactly $1-\eps$ and is pushed to a corner and the next hypersphere of radius $r$ is pushed to the diagonally opposite corner in the augmented bin. We claim that $r$ satisfies the form given above exactly. We use the Pythagorean theorem in $d$-dimensions repeatedly. The situation is described clearly in two dimensions in Figure \ref{hypersphere}.
	%\newpage
	\begin{figure}[ht]
		\centering
		\begin{tikzpicture}[scale=0.5]
		\coordinate (a) at (0,0);
		\coordinate (b) at (12,0);
		\coordinate (c) at (0,9);
		\coordinate (d) at (12,9);
		\coordinate (e) at (2,0);
		\coordinate (f) at (12-4.29,0);
		\draw (0,0) rectangle (12,9);
		\draw (2,2) circle (2cm);
		x=4;
		\draw (12-4.29,9-4.29) circle (4.29 cm);
		\draw[dashed] (2,2) -- (12,2);
		\draw [dashed] (12-4.29,0) -- (12-4.29,9);
		\draw [dashed] (2,2) -- (12-4.29,9-4.29);
		\draw [dashed] (2,0) -- (2,2);
		\draw [dashed] (0,2) -- (2,2);
		\draw (2,2) circle (2cm);
		\node[above left] at (2,2) {$O_2$};
		\node[above left] at (12-4.29,9-4.29) {$O_1$};
		\node[above left] at (12-4.29,2) {$P$};
		\draw[<->] ([yshift=-0.3cm]f) -- ([yshift=-0.3cm]b) node[midway, below]{$(1-\eps)/2$};
		\draw[<->] ([yshift=-0.3cm]a) -- ([yshift=-0.3cm]e) node[midway, below]{$r$};
		\label{Figure 4}
		\end{tikzpicture}
		\caption{Worst case scenario for second biggest sphere in two dimensions.}
		\label{hypersphere}
	\end{figure}
	%\newpage
	% \\\includegraphics[width=10cm]{Images/hypersphere.jpeg}
	
	Let a huge circle of the minimum diameter $1-\eps$ be pushed to the rightmost corner of the augmented box centered at $O_1$. We try and fit a circle of radius $r$ in the bottom-left corner of the box centered at $O_2$. We notice that in 2 dimensions, $O_1 O_2 P$ forms a right triangle. $O_2 P= 1+\eps - r - (1-\eps)/2$, $O_1 P = 1 - r - (1-\eps)/2$, and $O_1 O_2 = r + (1-\eps)/2$. Applying Pythagorean theorem in two dimensions, we get $r=\frac{3}{2} (1+\eps) - \sqrt(2+3\eps)$. In $d$-dimensions, this generalises to $r= \frac{1}{2}+\frac{1}{d-1}+\eps( \frac{1}{2} + \frac{2}{d-1}) -\sqrt{\frac{(1+\eps)^2}{(d-1)^2}+\frac{1-\eps^2}{d-1}}$ and we are done.
\end{proof}

%\begin{restatable}{lemma}{uniqhugeaabs}
\begin{lem}
	\label{uniqhuge}
	For any $0 < \eps \leqslant 1/2d^2$ for all $d \geqslant 2$, there can be at most one hypersphere in $P$ with a diameter larger than $1-\eps$.
	\end{lem}
%\end{restatable}
\begin{proof}
	We always get at most one \textit{huge} hypersphere if the radius calculated in the \Cref{nextrad} is always less than $(1-\eps)/2$. We show that such an $\eps>0$ can always exist regardless of $d$.
	\[\frac{1}{2}+\frac{1}{d-1}+\eps( \frac{1}{2} + \frac{2}{d-1}) -\sqrt{\frac{(1+\eps)^2}{(d-1)^2}+\frac{1-\eps^2}{d-1}} \leqslant (1-\eps)/2 \]
	Analytically solving the quadratic equation, it always holds for \[\eps \leqslant \frac{\sqrt{d^3+3d^2-4d+1}-d}{d^2+3d-1} \leqslant \frac{1}{2d^2}\] where the bound is always positive for all $d \geqslant 2$.
\end{proof}

%\begin{restatable}{theorem}{apxtheoremabs}
\begin{theorem}
	\label{3apx}
	There is a polynomial time $3$-approximation algorithm for the $\mathsf{d-CSK}$ problem.
	\end{theorem}
%\end{restatable}
\begin{proof}
	We show that for values of $\eps<1/2d^2$ as given in \Cref{uniqhuge} we can always partition the augmented bin packing $P$ into three separate packings into unit hypercube bins $B_1, B_2,$ and $B_3$. Let the unique huge hypersphere that intersects both $\ell$ and $\ell'$ be called $C_{huge}$ and remove $C_{huge}$ from all other types of hyperspheres in $P$ as defined earlier. If there is no \textit{huge} hypersphere, then ignore this step. Now note that the set of type 1, type 2, type 3, type 2', type 3', and $C_{huge}$ form a partition of the hyperspheres in $P$.  
	\\We first pack $B_1$ using the same structure as in $P$ with hyperspheres of type 3' and type 2'. This is possible as no hypersphere of type 2' can intersect $\ell$ and we can simply remove the $\eps$-slab to the right of $\ell'$ and we get our bin packing $B_1$. We then pack $B_3$ with hyperspheres of type 2, type 3, and type 1. We then pack the unique hypersphere $C_{huge}$ which has a diameter of at most 1 in a unit bin $B_2$. Note here that we needed to have at most one $C_{huge}$ as the bin width could have been more than 1 even though the huge hyperspheres themselves had a diameter less than 1. We then return the bin out of $B_1, B_2, B_3$ with the most profit.
	\\The running time of this algorithm is clearly polynomial as we get the augmented packing from \Cref{extended-wowa} in polynomial time and the partitioning takes linear time. 
	Since we return the bin with the maximum weight, we return a instance of $\mathsf{d-CSK}$ with a profit of at least $\frac{1}{3} w(\OPT)$. 
\end{proof}

\subsubsection{$(2+\eps)$-approximation algorithm for \(d\leq 8\)} \label{sec:appendix-2-apx}
The main goal of this section is to show that the packings we return for bins $B_1$ and $B_3$ in the $3$-approximation algorithms can in fact be packed into a single bin for $d\leqslant 8$. When there are no \textit{huge} hyperspheres with a diameter greater than $(1-\eps)$, a simple argument for packing in two bins can be made. Also, from \Cref{uniqhuge} we know that for small enough values of $\eps$, there can be at most one \textit{huge} hypersphere.

\begin{restatable}{lemma}{nohugelemmaapx}
	\label{nohuge}
	If there are no \textit{huge} hyperspheres with a diameter bigger than $1-\eps$, then the augmented bin packing $P$ can be partitioned into two unit bin packings $B_1$ and $B_2$.
\end{restatable}
\begin{proof}
	We partition using the same algorithm as in \Cref{3apx} into three unit bins. However the bin that contained the \textit{huge} hypersphere before is now completely empty, so we simply return the other two bins.
\end{proof}

If we have a unique \textit{huge} hypersphere $C_{huge}$, we again show that we can pack $P$ into two different unit bin packings $B_1$ and $B_2$. Let us define another $\eps$-slab $D$ which is parallel to $\ell$ and $\ell'$ and is situated exactly halfway between the two and has $\eps$-width. To use our strategy we need an "empty" $\eps$-slab $S$ in the middle of the augmented bin, which restricts the dimension to $d\leqslant 8$.


\begin{restatable}{lemma}{mindistlemma}
	\label{mindist}
	For $\eps < 1/d^2.2^d$ and $d \leqslant 8$, the distance between any arbitrary type 2 hypersphere and any arbitrary hypersphere of type 2' is at least $\eps$.
\end{restatable}
\begin{proof}
	If the diameter of the hypersphere calculated in \Cref{nextrad} is smaller than $1/2 - \eps$, this is true as the distance between $\ell$ and $D$, $\ell'$ and $D$ is $1/2 - \eps$.   
	\[\frac{1}{2}+\frac{1}{d-1}+\eps( \frac{1}{2} + \frac{2}{d-1}) -\sqrt{\frac{(1+\eps)^2}{(d-1)^2}+\frac{1-\eps^2}{d-1}} \leq 1/4 - \frac{\eps}{2}\]
	This inequality holds true for some positive value of $\eps$ only for $d\leq 8$.  
\end{proof}

\begin{restatable}{theorem}{approxtheorem}
	There is a polynomial time $(2+\eps)$-approximation algorithm for $\mathsf{d-CSK}$ for dimension $d<8$ and $0<\eps<1/4d^2.5^{2d+3}$.
\end{restatable}
\begin{proof}
	We choose $\eps$ small enough from \Cref{uniqhuge} such that there can be at most one \textit{huge} hypersphere of diameter bigger than $1-\eps$. Now, if there are no hyperspheres in the augmented packing $P$ obtained from  \Cref{extended-wowa} with a diameter bigger than $1-\eps$, we proceed to partition and pack $P$ into two augmented unit bins $B_1$ and $B_2$ using \Cref{nohuge}. 
	\\In the case where there is a unique \textit{huge} hypersphere, we choose $\eps$ small enough from \Cref{uniqhuge} such that type 2 and type 2' hyperspheres in $P$ leave an empty $\eps$-strip $D$ between them in the middle of the augmented bin. Now we pack the only huge hypersphere $C_{huge}$ and type 1 hyperspheres into $B_2$. We now can simply remove the strip $D$ and join the segments to get a unit bin packing $B_1$ of hyperspheres of types 2,3,2',3'.
	\\At the end we return packing out of $B_1,B_2$ with maximum weight. This algorithm is clearly polynomial as we get the augmented packing from \Cref{extended-wowa} in polynomial time and the partitioning takes linear time. The algorithm returns an instance of $\mathsf{d-CSK}$ of total weight at least of $\frac{(1-\eps)}{2}w(\OPT)$.
\end{proof}
\end{comment}
%%%%%%%%%
%%%%%%%%%%%


